Demystifying Visual Features of Movie Posters for Multi-Label Genre Identification

In the film industry, movie posters have been an essential part of advertising and marketing for many decades, and continue to play a vital role even today in the form of digital posters through online, social media and OTT (over-the-top) platforms. Typically, movie posters can effectively promote and communicate the essence of a film, such as its genre, visual style/tone, vibe and storyline cue/theme, which are essential to attract potential viewers. Identifying the genres of a movie often has significant practical applications in recommending the film to target audiences. Previous studies on genre identification have primarily focused on sources such as plot synopses, subtitles, metadata, movie scenes, and trailer videos; however, posters precede the availability of these sources, and provide pre-release implicit information to generate mass interest. In this paper, we work for automated multi-label movie genre identification only from poster images, without any aid of additional textual/metadata/video information about movies, which is one of the earliest attempts of its kind. Here, we present a deep transformer network with a probabilistic module to identify the movie genres exclusively from the poster. For experiments, we procured 13882 number of posters of 13 genres from the Internet Movie Database (IMDb), where our model performances were encouraging and even outperformed some major contemporary architectures.

==> 6_reference.tex <==
%\section*{References}

\begin{thebibliography}{27}
% \balance

% \bibitem{posner1976visual} Posner, M. I., Nissen, M. J., \& Klein, R. M. (1976). Visual dominance: An information-processing account of its origins and significance. Psychological Review, 83(2), 157–171. https://doi.org/10.1037/0033-295X.83.2.157

% \bibitem{howard1966human} Howard, I. P., \& Templeton, W. B. Human spatial
% orientation. New York: Wiley, 1966.

% \bibitem{merleau1962phenomenology} O'Regan, J., \& Noe, A. (2001). A sensorimotor account of vision and visual consciousness. Behavioral and Brain Sciences, 24(5), 939-973. doi:10.1017/S0140525X01000115

% \bibitem{abu2016youtube}	S. Abu-El-Haija, N. Kothari, J. Lee, P. Natsev, G. Toderici,
% B. Varadarajan, and S. Vijayanarasimhan. Youtube-8m:
% A large-scale video classification benchmark. CoRR,
% abs/1609.08675, 2016.

% \bibitem{agrawal2021color} Agrawal, Rishabh and Sivaprasad, Sarath and Pedanekar, Niranjan,Color Me Good: Branding in the Coloring Style of Movie Posters,Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops,
% June,
% 2021,
% 3899-3903

% \bibitem{hyland2002genre}Hyland, Ken. "Genre: Language, context, and literacy." Annual review of applied linguistics 22.1 (2002): 113-135.

% %\bibitem{8} XX
% %\bibitem{8} XX
% %\bibitem{8} XX
% %\bibitem{8} XX
% \bibitem{biber1986spoken} Biber, Douglas. "Spoken and written textual dimensions in English: Resolving the contradictory findings." Language (1986): 384-414.
% \bibitem{kessler-etal-1997-automatic} Automatic Detection of Text Genre (Kessler et al., ACL-EACL 1997)

% \bibitem{stamatatos2000automatic} Efstathios Stamatatos, Nikos Fakotakis, George Kokkinakis; Automatic Text Categorization in Terms of Genre and Author. Computational Linguistics 2000; 26 (4): 471–495. doi: https://doi.org/10.1162/089120100750105920

% \bibitem{stamatatos-etal-2000-text} E. Stamatatos, N. Fakotakis, and G. Kokkinakis. 2000. Text Genre Detection Using Common Word Frequencies. In COLING 2000 Volume 2: The 18th International Conference on Computational Linguistics.

% \bibitem{gorinski-lapata-2018-whats} What’s This Movie About? A Joint Neural Network Architecture for Movie Content Analysis (Gorinski \& Lapata, NAACL 2018)

% \bibitem{battu-etal-2018-predicting} Predicting the Genre and Rating of a Movie Based on its Synopsis (Battu et al., PACLIC 2018)

% \bibitem{kar-etal-2018-folksonomication} Folksonomication: Predicting Tags for Movies from Plot Synopses using Emotion Flow Encoded Neural Network (Kar et al., COLING 2018)

% \bibitem{kar-etal-2018-mpst} MPST: A Corpus of Movie Plot Synopses with Tags (Kar et al., LREC 2018)

% \bibitem{10.1145/3442381.3449806} Chen-Hsi Chang, Hung-Ting Su, Jui-Heng Hsu, Yu-Siang Wang, Yu-Cheng Chang, Zhe Yu Liu, Ya-Liang Chang, Wen-Feng Cheng, Ke-Jyun Wang, and Winston H. Hsu. 2021. Situation and Behavior Understanding by Trope Detection on Films. In Proceedings of the Web Conference 2021 (WWW '21). Association for Computing Machinery, New York, NY, USA, 3188–3198. https://doi.org/10.1145/3442381.3449806

% %\bibitem{8} XX

% \bibitem{10.1145/217279.215283} Stephan Fischer, Rainer Lienhart, and Wolfgang Effelsberg. 1995. Automatic recognition of film genres. In Proceedings of the third ACM international conference on Multimedia (MULTIMEDIA '95). Association for Computing Machinery, New York, NY, USA, 295–304. https://doi.org/10.1145/217279.215283

% \bibitem{truong2000automatic} Ba Tu Truong and C. Dorai, "Automatic genre identification for content-based video categorization," Proceedings 15th International Conference on Pattern Recognition. ICPR-2000, Barcelona, Spain, 2000, pp. 230-233 vol.4, doi: 10.1109/ICPR.2000.902901.

% \bibitem{1048494} Z. Rasheed and M. Shah, ”Movie genre classification by exploiting audio-visual fea-
% tures of previews,” 2002 International Conference on Pattern Recognition, Quebec
% City, QC, Canada, 2002, pp. 1086-1089 vol.2, doi: 10.1109/ICPR.2002.1048494.

% \bibitem{1377360} Z. Rasheed, Y. Sheikh and M. Shah, "On the use of computable features for film classification," in IEEE Transactions on Circuits and Systems for Video Technology, vol. 15, no. 1, pp. 52-64, Jan. 2005, doi: 10.1109/TCSVT.2004.839993.

% \bibitem{zhou2010movie} Howard Zhou, Tucker Hermans, Asmita V. Karandikar, and James M. Rehg. 2010.
% Movie genre classification via scene categorization. In Proceedings of the 18th ACM
% international conference on Multimedia (MM ’10). Association for Computing Ma-
% chinery, New York, NY, USA, 747–750. https://doi.org/10.1145/1873951.1874068


% \bibitem{Simes2016MovieGC} G. S. Simões, J. Wehrmann, R. C. Barros and D. D. Ruiz, "Movie genre classification with Convolutional Neural Networks," 2016 International Joint Conference on Neural Networks (IJCNN), Vancouver, BC, Canada, 2016, pp. 259-266, doi: 10.1109/IJCNN.2016.7727207.

% \bibitem{wehrmann2017movie} Jônatas Wehrmann, Rodrigo C. Barros,
% Movie genre classification: A multi-label approach based on convolutions through time,
% Applied Soft Computing,
% Volume 61,
% 2017,
% Pages 973-982,
% ISSN 1568-4946,
% https://doi.org/10.1016/j.asoc.2017.08.029.

% \bibitem{yadav2020unified} Ashima Yadav, Dinesh Kumar Vishwakarma,
% A unified framework of deep networks for genre classification using movie trailer,
% Applied Soft Computing,
% Volume 96,
% 2020,
% 106624,
% ISSN 1568-4946,
% https://doi.org/10.1016/j.asoc.2020.106624.

% \bibitem{4107177} X. Yuan, W. Lai, T. Mei, X. -s. Hua, X. -q. Wu and S. Li, "Automatic Video Genre Categorization using Hierarchical SVM," 2006 International Conference on Image Processing, Atlanta, GA, USA, 2006, pp. 2905-2908, doi: 10.1109/ICIP.2006.313037.

% \bibitem{brezeale2006using} Brezeale, Darin, and Diane J. Cook. "Using closed captions and visual features to classify movies by genre." Poster session of the seventh international workshop on Multimedia Data Mining (MDM/KDD2006). 2006.

% \bibitem{5204091} Van De Sande, Koen, Theo Gevers, and Cees Snoek. "Evaluating color descriptors for object and scene recognition." IEEE transactions on pattern analysis and machine intelligence 32.9 (2009): 1582-1596.

% \bibitem{rouvier2015audio}M. Rouvier, S. Oger, G. Linarès, D. Matrouf, B. Merialdo and Y. Li, "Audio-Based Video Genre Identification," in IEEE/ACM Transactions on Audio, Speech, and Language Processing, vol. 23, no. 6, pp. 1031-1041, June 2015, doi: 10.1109/TASLP.2014.2387411.

% \bibitem{8}XX

% \bibitem{8}XX

% \bibitem{8}XX



% \bibitem{10.1145/3019612.3019641} Jônatas Wehrmann and Rodrigo C. Barros. 2017. Convolutions through time for multi-label movie genre classification. In Proceedings of the Symposium on Applied Computing (SAC '17). Association for Computing Machinery, New York, NY, USA, 114–119. https://doi.org/10.1145/3019612.3019641

% \bibitem{deldjoo2018mmtf} Yashar Deldjoo, Mihai Gabriel Constantin, Bogdan Ionescu, Markus Schedl, and Paolo Cremonesi. 2018. MMTF-14K: a multifaceted movie trailer feature dataset for recommendation and retrieval. In Proceedings of the 9th ACM Multimedia Systems Conference (MMSys '18). Association for Computing Machinery, New York, NY, USA, 450–455. https://doi.org/10.1145/3204949.3208141

% \bibitem{10.1145/2827872} F. Maxwell Harper and Joseph A. Konstan. 2015. The MovieLens Datasets: History and Context. ACM Trans. Interact. Intell. Syst. 5, 4, Article 19 (January 2016), 19 pages. https://doi.org/10.1145/2827872

% \bibitem{huang2020movienet} Huang, Q., Xiong, Y., Rao, A., Wang, J., Lin, D. (2020). MovieNet: A Holistic Dataset for Movie Understanding. In: Vedaldi, A., Bischof, H., Brox, T., Frahm, JM. (eds) Computer Vision – ECCV 2020. ECCV 2020. Lecture Notes in Computer Science(), vol 12349. Springer, Cham. 

% \bibitem{cascante2019moviescope} Cascante-Bonilla, Paola, et al. "Moviescope: Large-scale analysis of movies using multiple modalities." arXiv preprint arXiv:1908.03180 (2019).

% \bibitem{montalvo2022trailers12k} Montalvo-Lezama, Ricardo, Berenice Montalvo-Lezama, and Gibran Fuentes-Pineda. "Trailers12k: Evaluating Transfer Learning for Movie Trailer Genre Classification." arXiv preprint arXiv:2210.07983 (2022).

% \bibitem{8}





































\end{thebibliography}

==> old/1intro.tex <==
\section{Introduction}\label{sec:intro}

\noindent
\IEEEPARstart{I}{n} 
% the contemporary landscape of the film industry, where digital platforms have revolutionized the way we consume content, the role of movie posters has undergone a profound transformation. These visual canvases, once primarily relegated to theater exhibits, newspaper ads, and DVD covers, have emerged as powerful tools for attracting audiences in the era of online streaming \cite{30_9057706}. 
% A movie poster is no longer just a piece of promotional artwork; it has become a gateway to a cinematic experience, a glimpse into the world of a film, and a crucial factor in a viewer's decision-making process.
% Beyond their aesthetic appeal, movie posters are rich repositories of information. They convey not only the visual aesthetics of a film but also subtle cues about its genre, style, and thematic content. A well-crafted poster can encapsulate the essence of a movie, enticing viewers with tantalizing glimpses of its narrative and emotional landscape. As viewers increasingly turn to online platforms to discover and enjoy films, movie posters have assumed a pivotal role in the digital realm, guiding users in their quest for cinematic satisfaction \cite{4_winoto2010role}.
%
the contemporary landscape of the film industry, 
digital platforms have revolutionized how content is consumed, elevating the role of movie posters. 
These visual canvases, once primarily relegated to theater exhibits, newspaper ads, and DVD covers, have emerged as powerful tools for attracting audiences in the era of online streaming \cite{30_9057706}. 
A movie poster is no longer just a piece of promotional artwork; it has become a gateway to a cinematic experience, a glimpse into the world of a film, and a crucial factor in a viewer's decision-making process.
Beyond their aesthetic appeal, posters convey subtle cues about the film's genre, style, and thematic content. A well-crafted poster can encapsulate the essence of a movie, enticing viewers with tantalizing glimpses of its narrative and emotional landscape. As viewers increasingly turn to online platforms to discover and enjoy films, movie posters have assumed a pivotal role in the digital realm, guiding users to their desired content \cite{4_winoto2010role}.

In the digital age, with the sheer volume of content available, accurate genre categorization is essential for audiences to navigate the extensive catalogs of online streaming platforms and find films that match their preferences \cite{netflix_frey2021}. 
The reliance on genre categorization underscores the crucial role of automated genre identification in improving film discoverability and enhancing the overall user experience. 
In the literature, while automated movie genre identification mostly used video trailers \cite{25_montalvo2022trailers12k,26_yadav2020unified} and textual plot synopses\cite{10_hoang2018predicting,13_wehrmann2018self},  
very few works engaged movie posters \cite{28_10.1145/3132515.3132516}. 
However, movie posters play a crucial role in genre identification, and subsequently attracting potential target audiences, since they precede the release of the film itself, even before trailers and synopses become available. 
Moreover, compared to the video/ textual modality, posters serve as prevalent thumbnails on OTT platforms, and are extensively shared across social media and various advertising/ promotional channels. 


% In the digital age, where the sheer volume of available content can be overwhelming, accurate genre categorization has become paramount. Audiences rely on genre labels to navigate the expansive catalogs of online streaming platforms, seeking films that resonate with their tastes and preferences \cite{netflix_frey2021}. 
% This reliance on genre categorization underscores the critical role that automated genre identification plays in enhancing the discoverability of films and improving the overall user experience.
%
% In the literature, automated movie genre identification has been performed mostly using video trailers \cite{25_montalvo2022trailers12k,26_yadav2020unified} and textual plot synopses\cite{10_hoang2018predicting,13_wehrmann2018self}. 
% A very few works have been reported using movie posters \cite{28_10.1145/3132515.3132516}. 
% However, movie posters play a crucial role in genre identification, and subsequently attracting potential target audiences, since they precede the release of the film itself, even before trailers and synopses become available. 
% Moreover, compared to the video/textual modality, posters serve as prevalent thumbnails on OTT platforms, and are extensively shared across social media and various advertising/ promotional channels. 
%
% This underscores the importance of poster designers in creating posters that accurately convey the film's genre. An automated genre identification system can assist designers in crafting and refining these posters. 
%
% This motivates us to undertake the task of genre identification solely from movie posters. 

\begin{figure}%[!h]
\centering
\scriptsize
\begin{tabular}{c|c|c|c}
% \hline 
% &&&   \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.2\linewidth, height=0.3\linewidth]{figs/challenge/2.jpg} & 
\includegraphics[width=0.2\linewidth, height=0.3\linewidth]{figs/challenge/7.jpg} & 
\includegraphics[width=0.2\linewidth, height=0.3\linewidth]{figs/challenge/27.jpg} & 
\includegraphics[width=0.2\linewidth, height=0.3\linewidth]{figs/challenge/9.jpg} \\  
\textcolor{blue}{{(a)}} drama, & \textcolor{blue}{{(b)}} action, & \textcolor{blue}{{(c)}} crime, & \textcolor{blue}{{(d)}} action,   \\
horror, mystery & sci-fi, \---  & mystery, thriller & adventure, fantasy \\
% \hline
\end{tabular}
\caption{Example of movie posters with genres}
\label{fig:intro_challenge}
\end{figure}


In Fig. \ref{fig:intro_challenge}, we present some movie poster samples with corresponding genres. 
Analyzing only poster images brings several challenges, since a single poster may have 
limited information (Fig. \ref{fig:intro_challenge}.(a)), 
intricate backgrounds (Fig. \ref{fig:intro_challenge}.(b)), 
incorporated multiple small images in a collage (Fig. \ref{fig:intro_challenge}.(c)), 
or included solely the cast member photos (Fig. \ref{fig:intro_challenge}.(d)). 
%
% Here, we analyze only the poster image without any aid of other modalities to identify its genre, which is a considerably more challenging task compared to other computer vision tasks, e.g., object detection, scene recognition and classification. 
% Unlike objects, genres are intangible implicit features that can hardly be precisely determined in a poster \cite{30_9057706}. 
We here analyze only the poster image without any aid of other modalities to identify its genre, considerably more challenging than other computer vision tasks, 
since genres are intangible implicit features and rely on individual human perception, i.e., 
% a poster may be classified as one genre by a person, but considered a different genre by another 
one person may classify a poster as one genre while another may classify it differently 
\cite{30_9057706}. 
Additionally, a poster can belong to multiple genres, introducing the challenge of multi-label classification \cite{Herrera2016} and potentially exacerbating data imbalance concerns \cite{Johnson2019SurveyOD}. 
In a poster, a genre may be suppressed by other genres, e.g., in Fig. \ref{fig:intro_challenge}.(d), \emph{action} and \emph{adventure} genres are more explicit than \emph{fantasy}. 
Moreover, the information present in a poster itself brings additional challenges in identifying the genre, which we briefly mention in Appendix \ref{app:data_challenge}. 
In this study, we procured posters from IMDb, where each poster can be multi-labeled \cite{Herrera2016} with up to three genres.


%%%%%%%%%%%%%%%%%%%%%%%%
% In this paper, our research goal is to effectively identify multi-label genres from a poster image, without any aid from textual, video, or audio modalities. 
% The primary motivation behind addressing this problem stems from the pivotal role that a poster plays on an OTT platform. The poster is often the first piece of content a user sees, which prompts them to click on the item to explore its content or watch the trailer, ultimately deciding whether they are interested in watching the movie. Therefore, it is crucial to design the poster in a way that effectively conveys the content or genre of the film. If the poster fails to do so, potential viewers interested in a particular genre might skip the movie, leading content creators to redesign the poster to better reflect its content. To address this need, an automated platform is necessary to determine whether a poster accurately identifies the genres. 
% However, identifying genres solely from a poster, without considering other modalities, is a relatively underexplored area in the literature. Previous research in this domain has not achieved satisfactory accuracy, often due to ineffective handling of the complexities of multi-label genre identification or by considering a limited number of genres. Therefore, the goal of this research is to effectively identify multiple genres from a poster image alone, without any textual, video, or audio inputs. To achieve this, we propose a novel approach incorporating several key techniques and contributions, as outlined below.


% In this paper, our research goal is to effectively identify multi-label genres from a poster image, without any aid from textual, video, or audio modalities. 
% The primary motivation behind addressing this problem stems from the pivotal role that a poster plays on an OTT platform. 

\textcolor{blue}{The primary motivation for addressing genre identification from posters lies in the pivotal role that a poster plays on OTT platforms. 
The poster is often the first piece of content a user sees, which prompts them to click on the item to explore its textual content or watch the trailer, ultimately deciding whether they are interested in watching the movie. 
Therefore, it is crucial to design the poster in a way that effectively conveys the content or genre of the film. 
If the poster fails to do so, potential viewers interested in a particular genre might skip the movie, leading content creators to redesign the poster to better reflect its content. 
To address this need, an automated system is necessary to determine whether a poster accurately identifies the genres. 
However, identifying genres solely from a poster, without considering other modalities, is a relatively underexplored area in the literature. 
Previous research in this domain has not achieved satisfactory accuracy, often due to ineffective handling of the complexities of multi-label genre identification or by considering a limited number of genres. 
Therefore, the goal of this paper is to effectively identify multiple genres from a poster image alone, without any aid from textual, video, or audio modalities.  
To achieve this, we propose a novel approach incorporating several key techniques and contributions, as outlined below:}  


\emph{\textbf{(i)} Novel model for understanding poster-genre relationships:} We propose a transformer-based architecture designed to comprehend the global context and intricate relationships between a poster and its multiple genres. We introduce a residual dense transformer model by leveraging densely connected transformer encoders that use deep feature embeddings as input instead of raw image patches \cite{dosovitskiy2020image}. This approach enhances the ability of the model to grasp global context and decipher complex visual relationships within the poster image.

\emph{\textbf{(ii)} Advanced multi-label classification technique:} To address the multi-label classification challenges inherent in posters associated with multiple genres, we introduce an ensemble technique combined with an asymmetric loss function. This method is particularly effective when positive labels are less prevalent than negative ones \cite{ridnik2021asymmetric}, improving the accuracy and reliability of genre predictions.

\emph{\textbf{(iii)} Probabilistic module for variable genre identification:} Our model includes a novel probabilistic module designed to handle the variability in the number of genres associated with each poster. This module aims to eliminate extraneous genres and accurately determine the correct number of genres, enhancing the precision of genre identification.

\emph{\textbf{(iv)} Extensive experiments and ablation studies:} We conducted comprehensive experiments on poster images obtained from IMDb to evaluate the effectiveness of our model. By comparing our approach with contemporary architectures and performing detailed ablation studies, we provide valuable insights into how visual elements of posters correlate with movie genres. These findings have significant implications for improving film recommendation systems and advancing the digital evolution of the film industry.


The rest of the paper is organized as follows. 
Section \ref{1_1sec:related} provides a concise overview of the related literature. 
The subsequent section \ref{3sec:method} discusses the proposed methodology, 
followed by section \ref{4sec:result}, which delves into the analysis of experimental results.
Finally, section \ref{5sec:conclusion} concludes this paper.

%%%%%%%%%%%%%%%%%%%%%%%


% \textcolor{blue}{In this paper, our research goal is to effectively identify multi-label genres from a poster image, without any aid from textual, video, or audio modalities. 
% To accomplish this, we propose a novel approach comprising several key techniques and contributions, as follows. 
% %
% We utilize a transformer-based architecture for its ability to grasp global context and decipher intricate relationships spanning the entire poster image \cite{dosovitskiy2020image}. 
% We first introduce a residual dense transformer model that involves densely connected transformer encoders using deep feature embeddings as input, instead of raw image patches. 
% %
% To tackle the multi-label classification challenge posed by posters associated with multiple genres, we employ an ensemble technique and adopt an asymmetric loss function, particularly when positive labels are less prevalent than negative ones \cite{ridnik2021asymmetric}. 
% %
% Furthermore, we introduce a probabilistic module to handle the variability in the number of genres associated with each poster, aiming to eliminate extraneous genres and accurately identify the correct number of genres. 
% %
% To assess the effectiveness of our model, we conducted comprehensive experiments on the poster images procured from IMDb, compared with contemporary architectures, and performed an ablation study. 
% Our findings provide valuable insights into the interplay between visual elements of posters and movie genres, offering potential benefits for film recommendation systems and the digital evolution of the film industry.} 




%====================================
% In this paper, we harness the power of a transformer-based architecture for its ability to grasp the global context and decipher intricate relationships spanning the entire poster image \cite{dosovitskiy2020image}. 
% We first introduce a residual dense transformer, and then engage an ensemble mechanism and an asymmetric loss to tackle multi-label genre identification \cite{ridnik2021asymmetric}. 
% Furthermore, we propose a probabilistic module to 
% accommodate a variable number of genres in the classification process. 
% We now briefly mention our \emph{\textbf{contributions}} to this paper. 

% \emph{\textbf{(i)}} 
% % We work with genre identification only from poster images without any aid from textual/ video/ audio modalities. 
% We introduce a residual dense transformer model, which features densely connected transformer encoders. 
% Here, the model takes deep feature embeddings as input, instead of raw image patches. 

% \emph{\textbf{(ii)}} 
% A poster can often be associated with multiple movie genres, presenting a multi-label classification challenge. To effectively address this issue, we employ an ensemble technique. Additionally, we adopt an asymmetric loss function to handle the intricacies of multi-label classification, particularly when positive labels are less prevalent than negative ones.

% \emph{\textbf{(iii)}} 
% Movie posters may exhibit a variable number of multi-genres. To adapt to this variability, we introduce a probabilistic module designed to eliminate extraneous genres and accurately discern the varying number of genres associated with each poster. To the best of our knowledge, this is the earliest attempt of its kind. 

% \emph{\textbf{(iv)}} 
% To assess the effectiveness of our model, we conducted comprehensive experiments on the poster images procured from IMDb, compared with contemporary architectures, and performed an ablation study.  
% Our findings offer valuable insights into the interplay between poster visual elements and movie genres, benefiting film recommendation systems and the film industry's digital evolution.





==> old/1related_old.tex <==
\section{Related Work}
\label{1_1sec:related}

% \input{tables/1relatedTable}

\input{tables/tab_related_new}

Our main focus in this paper is identifying multi-label movie genres exclusively from posters. 
Using only posters as input for this task is relatively limited in the literature \cite{}. 
However, some past works used trailer \cite{}, and facial frames \cite{} as visual inputs. 
Additionally, numerous studies have focused on textual inputs, such as movie synopses \cite{} and screenplays \cite{}. 
Furthermore, past research endeavors employed multimodal approaches, combining visual, textual, and audio data as input \cite{}. Now, we provide a concise overview of these prior investigations.

\subsection{Textual genre classification}

Movies have textual data such as synopsis, subtitle, etc. They provide a broader development of the story, encompassing major events that influence its course or noteworthy patterns of events. In today's world of the internet, many viewers write their reviews or experience of movies on social media. These textual data are useful for genre classification problems.  %which defines genres of movies.  

There has been done many research on movie genre classification based on synopsis \cite{ertugrul2018movie}, \cite{hoang2018predicting}, \cite{kar-etal-2018-folksonomication}, \cite{battu-etal-2018-predicting}, \cite{wehrmann2018self}. Ertugrul et al. \cite{ertugrul2018movie} first split movie plots into sentences and embedded them, then applied Bidirectional Long Short-Term Memory (BLSTM) to them. His studies show that BLSTM performs better than Logistic Regression (LR) and Recurrent Neural Networks (RNN). Naive Bayes (NB) with linguistic features, Extreme Gradient Boosting (XGBoost), and Gated Recurrent Unit (GRU) models used by Hoang \cite{hoang2018predicting}. Kar et al. \cite{kar-etal-2018-folksonomication} proposed a neural network modified on Convolutional Neural Network (CNN) and BLSTM and conducted experiments with on the Movie Plot Synopses with
Tags (MPST) corpus \cite{kar-etal-2018-mpst} and estimated a set of tags.  Battu \cite{battu-etal-2018-predicting} created a multi-language movie dataset and talked about CNN and Long Short-Term Memory (LSTM) based models to predict the genre and rating. Movie synopses were extracted from Labeled Movie Trailer Data (LMTD)  \cite{Simes2016MovieGC} and employed a self-attention-based framework to analyze it by Wehrmann \cite{wehrmann2018self}.
%Wehrmann et al. \cite{wehrmann2018self} retrieved synopsis from the LMTD-9 dataset  \cite{Simes2016MovieGC} and used self-attention-based architecture on it.
%In \cite{portolese2018use}, \cite{portolese2019exploring} Portoles used Conventional machine learning models such as Decision Tree (DT), Multi-Layer Perceptron (MLP), Binary Relevance (BR), Deep Back-Propagation Neural Network (DBPNN), Random k-Labelsets (RAKEL), Classifier Chains on synopses retrieved from TMDb\footnote{https://www.themoviedb.org/}. 
%Saputra \cite{saputra2019classification} also applied Multinomial Naive Bayes, Support Vector Machine (SVM), and MLP.

Some research has also been conducted where a synopsis is not utilized. 
%In \cite{Mukta_Khan_Ali_Mahmud_2017} Mukta retrieved IMDb users who have Twitter\footnote{https://twitter.com/} accounts and collected movie-reviewing tweets for those users. Using these tweets, he got users' personalities and values from the IBM Watson personality insight API\footnote{https://personality-insights-livedemo.mybluemix.net/} and further, he used NB, SVM, and Random Forest algorithm to identify users' movie genre preferences. 
Gorinski et al. \cite{gorinski-lapata-2018-whats} create a dataset from the jinni\footnote{http://www.jinni.com/.} database and employed LSTM-decoder-based architecture to predict movie attribute pairs such as mood, plot, genre, style, etc. from movie screenplay. 

% The first instance of applying the quantitative method to textual genre research was done by Biber et al. \cite{biber1986spoken} via using stylistic analysis variation in written and spoken text and presented a model which ranks genre from various textual features. Kessler et al. \cite{kessler-etal-1997-automatic} used logistic regression on lexical, structural, character-level, and derivative cues. Stamatatos et al. \cite{stamatatos2000automatic} \cite{stamatatos-etal-2000-text} performed text classification using multiple regression and discriminant analysis based on common word frequencies and stylistic differences among texts. Lee et al. \cite{lee2002text} worked on genre and subject-revealing features like lexical features and frequency of a term for a particular genre. Cosine similarity and Naive Bayes were applied to these features of the text. Long Short Term Memory (LSTM) decoder proposed by Gorinski et al. \cite{gorinski-lapata-2018-whats} to predict movie attributes such as genre, plot, mood, and overview from movie screenplay. Battu et al. \cite{battu-etal-2018-predicting} created a multi-language movie dataset and talked about Convolutional Neural Network (CNN) and LSTM-based models to predict the genre and rating of the movie from the synopsis. Kar et al. \cite{kar-etal-2018-folksonomication} proposed a neural network modified on CNN and BLSTM and conducted experiments with on the MPST dataset \cite{kar-etal-2018-mpst} and estimated a set of tags from movie synopses and the flow of emotions in the course of the plot. Chang et al. \cite{10.1145/3442381.3449806} presented Multi-Step Recurrent Relational Network(MSRRN) architecture which was based on BERT and GNN, it was examined on the proposed TiMoS dataset to understand situations and behavior from movie synopses by detecting tropes. Naive Bayes with linguistic features, XGBoost, and GRU models used by Hoang et al. \cite{hoang2018predicting} on the movie plot summaries. Ertugrul et al. \cite{ertugrul2018movie} first split movie plots into sentences and embedded them, then applied BLSTM to them. His studies show that BLSTM performs better than Logistic regression and Recurrent Neural Networks.  A person's actions in real life are influenced by his personality and values. Mukta et al. \cite{Mukta_Khan_Ali_Mahmud_2017} worked on this key theory in psychology and used it in movie genre classification. They have taken tweets from Twitter and analyzed the personality and values of users through IBM Watson personality insight. Further, they experimented and identified genres using personality, values, and both using Naive Bayes, Support Vector Machine (SVM), Random Forest, Random Tree, and RepTree. They only took 5 genres into consideration action, adventure, comedy, drama, and thriller.  

% https://www.sciencedirect.com/science/article/pii/S0923596510000172

%video scene/ poster work

\subsection{Visual genre classification}

Movies are visual content and it also has other visual data such as trailers, teasers, and posters. Scene, gesture or action of the person, lighting, motion, objects in the scene, and the way a person is speaking to someone in the movie provides cues about that movie's genre. 

Fisher \cite{10.1145/217279.215283} first started genre classification for videos. Numerous other works have subsequently followed it. %\cite{truong2000automatic}-[35].
Trailer is used in most of the research %\cite{1377360}, \cite{4412917}, 
\cite{zhou2010movie}, \cite{4107177}, %\cite{huang2012movie}, 
\cite{Simes2016MovieGC}, \cite{wehrmann2017movie},  \cite{10.1145/3019612.3019641}, \cite{yadav2020unified}, \cite{montalvo2022trailers12k}, and \cite{truong2000automatic}. 
%Rasheed \cite{1377360} used low-level visual features like shot detection, color variance, motion, lighting key without any text and audio cues, and learned genre via mean shift classification while \cite{4412917}, \cite{huang2012movie} applied DT and SVM respectively. 
Zhou et al. \cite{zhou2010movie} extracted keyframe features GIST, CENTRIST, and W-CENTRIST from trailers. To represent a movie, a beg of the visual word model was created and with that representation, movie similarity was calculated.
%K-Nearest Neighbors (KNN) classifier was used to classify a  trailer into one of the genres of drama, comedy, action, and horror.
The K-Nearest Neighbors (KNN) classifier was utilized to categorize a trailer into one of the genres of drama, comedy, action, and horror.
Paper \cite{4107177} is about applying the C4.5 DT to categorize video via temporal and spatial features of the video. A movie trailer dataset named LMTD consisting of 10000 movie trailers associated with 22 genres was developed by Simoes \cite{Simes2016MovieGC}. They used a subset of this dataset having 1067 movie trailers associated with 4 genres and performed their CNN-MoTion architecture to classify trailers into different genres. Wehrmann et al.\cite{wehrmann2017movie}\cite{10.1145/3019612.3019641} proposed convolutions through time (CTT) module on the LMTD-9 dataset to predict genre from trailers. In the paper \cite{yadav2020unified}, the researcher developed Emotional-based Genre Detection for Bollywood (EmoGDB) dataset containing 5 genres and 6 emotions and also developed an inception-LSTM-based model to detect genre and emotion. They performed cross-dataset validation with LMTD-9, Multifaceted Movie Trailer Feature (MMTF-14K) \cite{deldjoo2018mmtf}, Movielens ML-25 \cite{10.1145/2827872}. Montalvo-Lezama et al. \cite{montalvo2022trailers12k} collected 12000 movies and their metadata with 10 various genres and presented DIViTA, a transformer-based architecture to classify movies into genres using it.

There have been few works that use the movie poster and signals for genre identification. 
%\cite{ivasic2014movie}, \cite{ivasic2015automatic}, \cite{pobar2017multi}, \cite{10.1145/3132515.3132516}, \cite{8990490},  \cite{9057706}. 
Authors in 
%\cite{ivasic2014movie}, \cite{ivasic2015automatic}, 
\cite{pobar2017multi} used conventional machine learning algorithms like NB, RAKEL, and BR to predict multi-genre. Chu et al. \cite{10.1145/3132515.3132516} collected movie posters from IMDb and used CNN and You Only Look Once (YOLO) models to speculate genre from movie posters. The Turkish movie posters were collected in \cite{8990490} from the Centre of Turkish Cinema Studios and applied CNN-based architecture on it. Wi et al. \cite{9057706} employed a gram layer in CNN-based models as it extracted style features by applying a gram matrix on movie posters. 
% MEG brain signals were used as the feature by Ghaemmaghami et al. \cite{ghaemmaghami2015movie} and applied a Naive Bayes classifier to it. 



%Zhou et al. \cite{zhou2010movie} extracted keyframe features GIST, CENTRIST, and W-CENTRIST from trailers. To represent a movie, a beg of the visual word model was created and with that representation, movie similarity was calculated. KNN classifier was used to classify a  trailer into one of the genres of drama, comedy, action, and horror. Yuan et al.\cite{4107177} used the C4.5 decision tree to categorize video via temporal and spatial features of the video. Brezeale et al. \cite{brezeale2006using} used closed caption and discrete cosine transform (DCT) of movies to distinguish them into genres. The color descriptor is important for image and video recognition. Slightly change in light intensity and light color affects video categorization but alone color descriptors are not sufficient, as shown by Sande et al. \cite{5204091}.  Simoes et al.  \cite{Simes2016MovieGC} developed a movie trailer dataset named LMTD consisting of 10000 movie trailers associated with 22 genres. They used a subset of this dataset having 1067 movie trailers associated with 4 genres and performed their CNN-MoTion architecture to classify trailers into different genres. Wehrmann et al.\cite{wehrmann2017movie}\cite{10.1145/3019612.3019641} proposed convolutions through time (CTT) module on the LMTD-9 dataset to predict genre from trailers. Ashima et al. \cite{yadav2020unified} developed Emotional-based Genre Detection for Bollywood (EmoGDB) dataset containing 5 genres and 6 emotions, and also developed an inception-LSTM-based model to detect genre and emotion. They performed cross-dataset validation with LMTD-9, Multifaceted Movie Trailer Feature (MMTF-14K) \cite{deldjoo2018mmtf}, Movielens ML-25 \cite{10.1145/2827872}.  Chu et al. \cite{10.1145/3132515.3132516} collected movie posters from IMDb and used CNN and YOLO models to speculate genre from movie posters. The Turkish movie posters were collected by Gozuacik et al. \cite{8990490} from the Centre of Turkish Cinema Studios and applied CNN-based architecture to it. Wi et al. \cite{9057706} applied a gram layer in CNN-based models as it extracted style features by applying a gram matrix on movie posters. MEG brain signals were used as the feature by Ghaemmaghami et al. and applied a Naive Bayes classifier to it \cite{ghaemmaghami2015movie}.  Montalvo-Lezama et al. \cite{montalvo2022trailers12k} collected 12000 movies and their metadata with 10 various genres and presented DIViTA architecture to classify movies into genres using it. 
%Sung et al. attempt to predict genre from movie posters via CNN architecture in the Standford project.
% hybrid/ muti-modal

\subsection{Multimodal genre classification}
Two or more features from the textual, visual, and audio features are being used in multimodal data.
%Rasheed \cite{1048494} used average shot length and motion content to classify the preview (trailer) of the movies into action and non-action. 
Average shot length and motion content were employed by Rasheed \cite{1048494} to classify movie previews (trailers) into either action or non-action categories.
%Based on the light intensity, non-action movies were further classified into comedy, horror, drama/others. Action movies were examined more based on audio features and explosion detection. 
Using light intensity as a criterion, non-action movies were additionally categorized as comedy, horror, and drama/others. Action movies go through more detailed assessment, focusing on audio features and detecting explosions.
Authors in \cite{brezeale2006using} used closed caption (subtitle) and discrete cosine transform (DCT) of the trailer and further applied SVM on it.
%Audio features such as interactivity, audio quality, and visual features like color, shape, shot, and foreground segmentation from videos were used by Rouvier et al. \cite{rouvier2015audio}, and proposed feature fusion and SVM classifier to speculate genres. 
In \cite{huang2020movienet} Huang developed the MovieNet dataset consisting of reach annotations of  1100 movies. They performed a wide range of experiments on it for better movie understanding and employed ResNet50, Temporal Relation Network (TRN) \cite{zhou2018temporal} for genre analysis. Cascante-Bonilla et al. \cite{cascante2019moviescope} proposed Moviescope, a multiple modalities dataset containing trailers, posters, plots, and metadata, and used the multimodel fusion technique to make use of it. In %\cite{ekenel2013multimodal}
\cite{mangolin2022multimodal} proposed a fusion of textual feature, LSTM and CNN-based architectures
%multimodal approach 
to detect genre from video, poster, text, and audio. Arevalo \cite{arevalo2017gated} proposed Gated Multimodal Units (GMU) to fuse data and employed CNN-based architecture top of GMU to identify genre via poster, synopsis, and metadata. Authors in \cite{bribiesca2021multimodal} applied a transformer-based model with GMU on posters, videos, audio, synopsis, and metadata. 
 %In \cite{hong2015multimodal} Hong used probabilistic latent semantic analysis  (PLSA) on video, audio, and textual data. Fu et al.  \cite{fu2015fast} used SVM to detect genre from posters and synopsis. 

%Multiple genres can be associated with a movie. Detecting multiple objects in the frame is a difficult task. Recently, Multilabel classification is an interesting research area as computational power increased drastically.

Our work is one of the earlier attempts to identify genre from only the visual features of movie posters using transformer architecture. At the time of research, we found datasets are publicly unavailable. Therefore, we created a dataset by manually checking after crawling posters from the IMDb website. We proposed ViT-based architecture and conducted extensive experiments on data.












==> old/4result.tex <==
\section{Experiments and Discussion}
\label{4sec:result}

%\noindent
% This section presents the employed dataset followed by experimental results and ablation study with discussions.
This section describes the employed dataset, followed by experimental details, evaluation metrics, model performance, and comparisons.
%, ablation studies, and discussions.

%\subsection{Database Employed}
\subsection{Employed Dataset}
\label{subsec:DB}

\input{2_dataset}

As previously stated in \autoref{2sec:challenge}, we procured a total of 13882 distinct posters, each considering up to 3 genres among a pool of 13 genres to perform experimental analysis. 
The ground-truth genre of a movie poster is available in terms of multi-hot encoding (refer to \autoref{subsec:prob_form}). 
% The ground truth label is converted using a multi-hot encoding vector. 
% We resized each poster to $1024 \times 1024$. 
%
The dataset was split up into training ($DB_{tr}$), validation ($DB_v$), and testing ($DB_t$) sets with an approx ratio of $8:1:1$ considering the presence of all 13 genres in each set equivalently.
$DB_{tr}$, $DB_v$, and $DB_t$ contain 10942, 1470, and 1470 posters, respectively. 
As a matter of fact, no common poster is present in $DB_{tr}$, $DB_v$, and $DB_t$.


\subsection{Experimental Details}
\label{subsec:Exp_details}

% In this subsection, we talk about our performed experiments and results to analyze the effectiveness of the proposed architecture. 
In this subsection, we present the experiments conducted to evaluate the effectiveness of the proposed architecture and discuss the results obtained. 

We executed the experimentation using the TensorFlow framework-2.5 having Python 3.9.13 over Ubuntu 20.04.2 LTS OS-based machine with the following configurations: AMD EPYC 7552 Processor @ 2.20 GHz with 48 CPU cores and 256 GB RAM, NVIDIA A100-PCIE with 40 GB memory.
In this paper, all the presented results were obtained from $DB_t$.

 
The hyper-parameters of our architecture were adjusted and set while the training of the model over the performance of $DB_v$. 
For all the transformer networks, we fix the following hyper-parameters empirically: 
transformer\_layers ($L$) = 4, 
embedding\_dimension ($D$) = \textcolor{red}{256}, %384? or 
num\_heads ($h$) = 6.
In Adam optimizer, we chose 
initial\_learning\_rate = $10^{-3}$; 
exponential decay rates for 1$^{st}$ and 2$^{nd}$ moment estimates, i.e., $\beta1=0.9$, $\beta2=0.999$; 
zero-denominator removal parameter ($\upvarepsilon$) = $10^{-8}$. 
For early stopping, we fixed the patience as 10 epochs. 
The mini-batch size was fixed to 32.



\subsection{Evaluation Metrics}
\label{subsec:Eval_metrics}

Movie genre identification is a multi-label classification problem \cite{Herrera2016}, thus the model performance has been evaluated through a macro analysis of the following
\cite{eval_method1, eval_method2}: $Precision$, $Recall$, $F_1-Measure$, $Accuracy$, $Balanced Accuracy$, $Specificity$, and $hamming Loss$. In macro analysis, firstly compute these measures independently for each class label and then take the average of all classes, which Resultant, $Precision_{macro}$, $Recall_{macro}$, $F_1-Measure_{macro}$, $Accuracy_{macro}$, $Balanced Accuracy_{macro}$, $Specificity_{macro}$, and $Hamming Loss$. Let the dataset consist of $n$ multi-label samples ($x_i, Y_i$) and let $h(.)$ multilabel classifier then four basic quantities of performance true positive ($TP$), false positive ($FP$), true negative ($TN$) and false negative ($FN$) for $j^{th}$ class label $y_j$ defined as:

\begin{equation}\label{eq:eq22}
\begin{split}
    TP_j = |\{x_i : y_j \in Y_i  \land  y_j \in h(x_i)\},1\leq i\leq n| \\
    FP_j = |\{x_i : y_j \notin Y_i  \land  y_j \in h(x_i)\},1\leq i\leq n| \\
    TN_j = |\{x_i : y_j \notin Y_i  \land  y_j \notin h(x_i)\},1\leq i\leq n| \\
    FN_j = |\{x_i : y_j \in Y_i  \land  y_j \notin h(x_i)\},1\leq i\leq n| 
\end{split}
\end{equation}

Naturally from this definition of equation \ref{eq:eq22}, $TP_j +FP_j + TN_j + FN_j = n$ always holds true. Further, We calculated $j^{th}$ class label and overall macro analysis of models using the following evaluation metrics :

\begin{equation}
\begin{split}
    Precision_j, {\cal{P}}_j = \frac{TP_j}{TP_j+FP_j}\\
    Precision_{Macro}, {\cal{P}} =\frac{\sum_{j=1}^{V} {\cal{P}}_j}{V} 
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
    Recall_j, {\cal{R}}_j = \frac{TP_j}{TP_j+FN_j} \\
    Recall_{Macro}, {\cal{R}} =\frac{\sum_{j=1}^{V} {\cal{R}}_j}{V} 
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
    Accuracy_j, {\cal{A}}_j = \frac{TP_j+TN_j}{TP_j+FP_j+TN_j+FN_j} \\
    Accuracy_{Macro}, {\cal{A}} =\frac{\sum_{j=1}^{V} {{\cal{A}}_j}}{V} 
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
    F_1-Measure_j, {\cal{FM}}_j = \frac{2 \times {\cal{P}}_j \times {\cal{R}}_j}{{\cal{P}}_j + {\cal{R}}_j} \\
    F_1-Measure_{Macro}, {\cal{FM}} =\frac{\sum_{j=1}^{V} {\cal{FM}}_j}{V} 
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
   Specificity_j, {\cal{S}}p_j = \frac{TN_j}{TN_j+FP_j} \\
    Specificity_{Macro}, {\cal{S}}p =\frac{\sum_{j=1}^{V} {\cal{S}}p_j}{V} 
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
    Balanced Accuracy_j, {\cal{BA}}_j = \frac{{\cal{R}}_j + {\cal{S}}p_j}{2} \\
    Balanced Accuracy_{Macro}, {\cal{BA}} =\frac{\sum_{j=1}^{V} {\cal{BA}}_j}{V} 
    \end{split}
\end{equation}

Where $V$ is the total number of genre categories. As mentioned in \autoref{subsec:DB}, In our case $V=13$. The Hamming Loss quantifies the average count of inaccurate predictions made regarding the relevance of an example to a class label \cite{eval_method2}. It is defined as below:

\begin{equation}
    % Hamming Loss, {\cal{HL}} = \frac{\sum_{i=1}^{n}\frac{h(x_i) \delta Y_i}{V}}{n}
    Hamming Loss, {\cal{HL}} = \frac{1}{n} \sum_{i=1}^{n} \frac{1}{V} | h(x_i) \Delta Y_i |
\end{equation}
Where $\Delta$ indicates the symmetric difference between
two sets.




% \begin{equation}
%     \begin{split}
%     Precion_j ({\cal{P}}_j) = \frac{TP_j}{TP_j+FP_j} \\
%     Recall_j ({\cal{R}}_j) = \frac{TP_j}{TP_j+FN_j} \\
%     Accuracy_j ({\cal{A}}_j) = \frac{TP_j+TN_j}{TP_j+FP_j+TN_j+FN_j} \\
%     F1-Measure_j ({\cal{FM}}_j) = \frac{2 \times {\cal{P}}_j \times {\cal{R}}_j}{{\cal{P}}_j + {\cal{R}}_j} \\
%     Specificity_j ({\cal{S}}p_j) = \frac{TN_j}{TN_j+FP_j} \\
%     Balanced Accuracy_j ({\cal{BA}}_j) = \frac{{\cal{R}}_j + {\cal{S}}p_j}{2}
%     \end{split}
% \end{equation}

\input{4resultTable}




\subsection{Model Performance}
% \label{subsec:results}
\label{subsec:model_perform}
We present the performance of the proposed RVD and PrRVD with respect to evaluation metrics mentioned in \autoref{subsec:Eval_metrics}. From \autoref{tab:tab3}, We observe both models performed well in movie multi-genre identification.

\subsubsection{\textbf{Various Ensemble Models}} 
In \autoref{tab:tab4}, we present the performance of the various ensembled models using multiple combinations of the proposed model. Here, RVD + RV + VD performed significantly better than other ensembled models in terms of $Precision_{macro}$, $Accuracy_{macro}$, and $Hamming Loss$ for both without probability and with probability. RVD + RV also achieves the best $Recall_{macro}$, and  $F_1-Measure_{macro}$. 

\subsubsection{\textbf{Genre Wise Analysis}}
\autoref{tab:genre_RVD}, \ref{tab:genre_RVD_RV_VD}, \ref{tab:genre_RVD_RV} present individual genre wise performance of RVD, RVD + RV + VD, RVD + RV for both without probability and with probability. We can observe that these 3 models identify the animation genre most accurately and performed well for action, adventure, comedy, and drama genres. They struggle to identify biography, fantasy, and mystery correctly. One of the reasons to struggle with these genres is they have less number of movie posters as mentioned in \autoref{2sec:challenge}. 

The performance of the RVD, RVD + RV + VD, and RVD + RV models according to the number of genres associated with the movie demonstrated in \autoref{tab:genre_ALL}. The table shows the performance of models improves as the number of genres increases. This is happening because of the imbalanced data with respect to the number of genres associated with the movie, which is shown in \autoref{fig:movie_poster_count}.b. For a single genre or 1 genre, RVD + RV + VD dominated and it performed overall better than the rest two models.



% \begin{table}[]
%     \centering
%     \caption{Caption}
% % \begin{adjustbox}{width=0.5\textwidth}    
%     \begin{tabular}{ c|c | c |c}
%     \hline
%        \textbf{Architecture}  & \multicolumn{3}{c}{\textbf{Accuracy (\%)}} \\ \cline{2-4}
%          & HA@1 & HA@2 & HA@3 \\
%     \hline\hline
%     ResNet50 \cite{he2016deep} & 72.24 & 54.49 & 43.67\\
%     DenseNet121 \cite{8099726} & 48.16 & 25.10 & 21.77\\
%     EfficientNetB2 \cite{tan2019efficientnet} & 71.82 & 55.10 & 43.53\\
%     ViT \cite{dosovitskiy2020image} & 46.25 & 44.63 & 35.85\\
%     Ours & \textbf{76.19} & \textbf{59.62} & \textbf{49.54}\\
%     \hline
%     \end{tabular}
% % \end{adjustbox}
    
%     \label{tab2}
% \end{table}

% \begin{table*}[]
%     \centering
%     \caption{Precision comparison of the Top-3 genres.}% without probability
%     \begin{adjustbox}{width=1\textwidth} 
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        ResNet50 \cite{he2016deep} & 0.66 & 0.66 & 0.87 & 0.21 & 0.60 & 0.46 & 0.57 & 0.36 & 0.50 & 0.41 & 0.48 & 0.56 & 0.43 & 0.57 & 0.52 \\

%          \hline
%        DenseNet121 \cite{8099726} & 0.36 & 0.50 & 0.17 & 0.05 & 0.47 & 0.50 & 0.49 & 0 & 0.30 & 0 & 0.12 & 0.20 & 0.24 & 0.32 & 0.26  \\
%        \hline
%        EfficientNetB2 \cite{tan2019efficientnet} & 0.70 & 0.73 &  0.84 & 0.24 & 0.62 & 0.43 & \textbf{0.60} & 0.24 & 0.54 & 0.31 & 0.48 & 0.48 & 0.46 & 0.57 & 0.51 \\

%          \hline
%        ViT \cite{dosovitskiy2020image} & 0.47 & 0.37 & 0 & 0 & 0.46 & 0.29 & 0.45 & 0.18 & 0.35 & 0.30 & 0.33 & 0.25 & 0.34 & 0.42 & 0.29  \\

%        \hline
%        Ours & \textbf{0.75} & \textbf{0.73} & \textbf{0.95} & \textbf{0.30} & \textbf{0.63} & \textbf{0.53} & 0.58 & \textbf{0.65} & \textbf{0.68} & \textbf{0.38} & \textbf{0.54} & \textbf{0.69} & \textbf{0.49} & \textbf{0.63} & \textbf{0.61}\\
%        \hline
%     \end{tabular}
%     \end{adjustbox}
    
%     \label{tab3}
% \end{table*}


% \begin{table*}[]
%     \centering
%     \caption{Recall comparison of the Top-3 genres.}%  without probability
%     \begin{adjustbox}{width=1\textwidth} 
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller}  & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        ResNet50 \cite{he2016deep} & 0.73 & 0.67 & 0.80 & 0.04 & 0.75 & 0.45 & 0.88 & 0.05 & 0.53 & 0.26 & 0.58 & 0.29 & 0.54 & \textbf{0.61} & \textbf{0.50} \\

%          \hline
%        DenseNet121 \cite{8099726} & 0.16 & 0.10 & 0.09 & 0.07 & 0.77 & 0.01 & 0.93 & 0 & 0.34 & 0 & 0.79 & 0.24 & 0.03 & 0.34 & 0.27  \\
%        \hline
%        EfficientNetB2 \cite{tan2019efficientnet} & 0.74 & 0.68 & \textbf{0.82} & \textbf{0.11} & 0.69 & \textbf{0.57} & 0.81 & \textbf{0.25} & \textbf{0.52} & \textbf{0.33} & 0.56 & \textbf{0.32} & 0.45 & 0.61 & 0.53  \\

%          \hline
%        ViT \cite{dosovitskiy2020image} &  \textbf{0.80} & 0.72 & 0 & 0 & 0.53 & 0.06 & \textbf{0.98} & 0.06 & 0.21 & 0.03 & 0.01 & 0.01 & 0.14 & 0.45 & 0.27 \\


%        \hline
%        Ours & 0.71 & \textbf{0.72} &0.73 & 0.06 & \textbf{0.78} & 0.46 & 0.89 & 0.07 & 0.43 & 0.23 & \textbf{0.59} & 0.24 & \textbf{0.46} & 0.60 & 0.49\\
%        \hline
%     \end{tabular}
% \end{adjustbox}
    
%     \label{tab4}
% \end{table*}


% \textbf{Genre hit accuracy}:  In Tables \ref{tab2}, we present the performance of our architecture and compare it to some advanced deep learning-based techniques. We got 76.19\%, 59.22\%, and 45.44\% hit accuracy for $1^{st}$, $2^{nd}$, and $3^{rd}$ genre detection respectively.  From the table It can be observed, our model outperformed major methods. Res-ViT-Dense obtained the second-best performance of 74.69\% and 58.37\% hit accuracy for 1st and 2nd genre detection and performed best in 3rd genre detection with 48.07\% hit accuracy.

%\textbf{Top-3 genre without probability}:

% \textbf{Top-3 genre with probability}:
% Now, we discuss the performances of architecture for each genre. As mentioned earlier, our dataset contains 13 genres. Table \ref{tab3}, \ref{tab4} presents each genre's precision and recall. We got the best precision of 0.94 for animation through ResNet50 and the best recall of 0.98 for drama through Vit and ViT-Dense. Overall Res-VIT-Dense performed best with the highest micro average, macro average precision, and recall respectively 0.59, 0.58, 0.63, 0.55. We also observed that every model struggled to detect biography and fantasy genres.

% \textbf{Biography binary classification}: 
% As observed models were poorly performed for biography, we further analyzed it. We manually select non-biography posters and created a subset by choosing 1076 biography and 1076 non-biography posters from the dataset. We build a binary classification model using ResNet50 on this subset. 
% The input is a $1024 \times 1024$ sized image and the output is $0$ for non-biography and $1$ for biography. As shown in Table \ref{tab5}, ResNet50 obtained 0.53 precision, 0.69 recall, and 57.87\% accuracy. We noticed that detecting biography is tough in our dataset.




% \begin{table*}[]
%     \centering
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c |c|c|}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        ResNet50 \cite{he2016deep}  & 0.69 & 0.62 & \textbf{0.94} & 0 & 0.55 & 0.39 & 0.53 & 0 & 0.65 & 0.34 & 0.37 & 0.61 & 0.41 & 0.53 & 0.47 \\

%          \hline
%        DenseNet121 \cite{8099726} & 0.36 & 0.50 & 0.18 & 0.05 & 0.47 & \textbf{0.50} & 0.49 & 0 & 0.30 & \textbf{0.50} & 0.12 & 0.19 & 0.24 & 0.32 & 0.30 \\
%        \hline
%        EfficientNetB2 \cite{tan2019efficientnet} & 0.70 & 0.72 & 0.89 & \textbf{0.38} & 0.60 & 0.43 & 0.58 & 0.26 & 0.58 & 0.34 & \textbf{0.47} & 0.52 & \textbf{0.47} & 0.57 & 0.53 \\

%          \hline
%        ViT \cite{dosovitskiy2020image} & 0.47 & 0.34 & 0 & 0 & 0.41 & 0.25 & 0.44 & 0.40 & 0.37 & 0.27 & 0.23 & 0.50 & 0.32 & 0.40 & 0.31\\

%        \hline
%        Res-ViT & 0.73 & 0.66 & 0.92 & 0.24 & 0.64 & 0.45 & \textbf{0.61} & 0.44 & 0.60 & 0.36 & 0.45 & 0.46 & 0.46 & 0.58 & 0.54  \\
%        \hline
%        ViT-Dense & 0.53 & 0.49 & 0.09 & 0 & 0.31 & 0.24 & 0.44 & 0 & 0.32 & 0.18 & 0.17 & 0.50 & 0.31 & 0.35 & 0.28  \\

%          \hline
%        Res-ViT-Dense & \textbf{0.78} & \textbf{0.78} & 0.89 & 0.33 & \textbf{0.70} & 0.43 & 0.57 & \textbf{0.53} & 0.63 & 0.37 & 0.46 & 0.68 & 0.44 & \textbf{0.59} & \textbf{0.58}  \\

%        \hline
%        Ours & 0.75 & 0.66 & 0.86 & 0 & 0.56 & 0.43 & 0.51 & 0 & \textbf{0.71} & 0.37 &0.42 & \textbf{0.77} & 0.43 & 0.55 & 0.50\\
%        \hline
%     \end{tabular}
%     \caption{Precision comparison of the Top-3 genres with probability.}
%     \label{tab3}
% \end{table*}


% \begin{table*}[]
%     \centering
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c |c|c |}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        ResNet50 \cite{he2016deep}  & 0.66 & 0.70 & 0.45 & 0 & 0.77 & 0.47 & 0.93 & 0 & 0.29 & 0.22 & 0.66 & 0.09 & 0.51 & 0.57 & 0.44 \\

%          \hline
%        DenseNet121 \cite{8099726} & 0.16 & 0.10 & 0.07 & 0.08 & 0.78 & 0.01 & 0.93 & 0 & 0.34 & 0 & \textbf{0.80} & 0.22 & 0.03 & 0.34 & 0.27  \\
%        \hline
%        EfficientNetB2 \cite{tan2019efficientnet} & \textbf{0.75} & 0.71 & 0.72 & 0.09 & 0.74 & 0.59 & 0.87 & \textbf{0.14} & 0.44 & 0.31 & 0.59 & 0.28 & 0.46 & 0.61 & 0.51 \\

%          \hline
%        ViT \cite{dosovitskiy2020image} & 0.72 & 0.21 & 0 & 0 & 0.72 & 0.41 & \textbf{0.98} & 0.01 & 0.10 & 0.04 & 0.32 & 0.01 & 0.10 & 0.42 & 0.28 \\

%        \hline
%        Res-ViT & 0.70 & 0.75 & 0.76 & 0.15 & 0.77 & 0.53 & 0.81 & 0.10 & 0.48 & \textbf{0.43} & 0.67 & \textbf{0.41} & 0.46 & 0.62 & 0.54 \\
%        \hline
%        ViT-Dense & 0.34 & 0.13 & 0.01 & 0 & \textbf{0.95} & 0.32 & \textbf{0.98} & 0 & 0.07 & 0.04 & 0.54 & 0.01 & 0.04 & 0.37 & 0.26 \\

%          \hline
%        Res-ViT-Dense & 0.64 & 0.66 & \textbf{0.78} & \textbf{0.19} & 0.71 & \textbf{0.65} & 0.90 & 0.06 & \textbf{0.54} & \textbf{0.43} & 0.71 & 0.32 & \textbf{0.58} & \textbf{0.63} & \textbf{0.55} \\

%        \hline
%        Ours & 0.73 & \textbf{0.75} & 0.07 & 0 & 0.82 & 0.48 & 0.93 & 0 & 0.39 & 0.28 & 0.70 & 0.11 & 0.53 & 0.59 & 0.44\\
%        \hline
%     \end{tabular}
%     \caption{Recall comparison of the Top-3 genres with probability.}
%     \label{tab4}
%\end{table*}





% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%     \hline
%        Evaluation matrix  & ResNet50 \cite{he2016deep}\\
%        \hline\hline
%         Precision & 0.53\\
%         Recall & 0.69\\
%         Accuracy (\%) & 57.87\\
%         \hline
%     \end{tabular}
%     \caption{Experimental result of biography and non-biography binary classification }
%     \label{tab5}
% \end{table}





% \subsection{Ablation Studies}
% \begin{table}[]
%     \centering
%     \caption{Caption}
%     \begin{tabular}{ c|c | c |c}
%     \hline
%        \textbf{Architecture}  & \multicolumn{3}{c}{\textbf{Accuracy (\%)}} \\ \cline{2-4}
%          & HA@1 & HA@2 & HA@3 \\
%     \hline\hline
%     Res-ViT & 74.62 & 57.48 & 42.78\\
%     ViT-Dense & 43.27 & 38.78 & 36.46\\
%     Res-ViT-Dense & 74.69 & 58.37 &  48.07\\
%     Ours(without probability) & \textbf{76.19} & 59.22 & 45.44 \\
%     Ours(with probability) & \textbf{76.19} & \textbf{59.62} & \textbf{49.54}\\
%     \hline
%     \end{tabular}
    
%     \label{tab2}
% \end{table}


% \begin{table*}[]
%     \centering
%     \caption{Precision comparison of the Top-3 genres.}% without probability
%     \begin{adjustbox}{width=1\textwidth} 
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        Res-ViT  & 0.75 & 0.67 & 0.87 & 0.18 & 0.66 & 0.46 & \textbf{0.63} & 0.29 & 0.59 & 0.36 & 0.45 & 0.44 & 0.46 & 0.58 & 0.53  \\
%        \hline
%        ViT-Dense & 0.46 & 0.44 & 0.43 & 0 & 0.32 & 0.29 & 0.44 & 0 & 0.29 & 0.15 & 0.21 & 0.30 & 0.40 & 0.39 & 0.29 \\

%          \hline
%        Res-ViT-Dense  & \textbf{0.76} & \textbf{0.82} & 0.86 & 0.27 & \textbf{0.74} & 0.43 & 0.60 & 0.36 & 0.54 & 0.37 & 0.52 & 0.55 & 0.47 & 0.59 & 0.56 \\
%        \hline
%        Ours & 0.75 & 0.73 & \textbf{0.95} & \textbf{0.30} & 0.63 & \textbf{0.53} & 0.58 & \textbf{0.65} & \textbf{0.68} & \textbf{0.38} & \textbf{0.54} & \textbf{0.69} & \textbf{0.49} & \textbf{0.63} & \textbf{0.61}\\
%        \hline
%     \end{tabular}
%     \end{adjustbox}
    
%     \label{tab3}
% \end{table*}


% \begin{table*}[]
%     \centering
%     \caption{Recall comparison of the Top-3 genres.} %  without probability
%     \begin{adjustbox}{width=1\textwidth} 
%     \begin{tabular}{| c| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
%       \hline \backslashbox{Methods}{Genres}  &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller}  & \rotatebox[origin=c]{90}{Micro avg.} & \rotatebox[origin=c]{90}{Macro avg.}\\
%       \hline \hline
%        Res-ViT  & 0.68 & \textbf{0.75} & \textbf{0.87} & 0.17 & 0.76 & 0.52 & 0.78 & 0.14 & 0.54 & \textbf{0.43} & \textbf{0.61} & \textbf{0.52} & 0.45 & 0.62 & 0.56 \\
%        \hline
%        ViT-Dense & \textbf{0.74} & 0.08 & 0.16 & 0 & \textbf{0.92} & 0.03 & \textbf{0.99} & 0 & 0.26 & 0.03 & 0.30 & 0.02 & 0.02 & 0.41 & 0.27  \\

%          \hline
%        Res-ViT-Dense & 0.67 & 0.62 & \textbf{0.87} & \textbf{0.37} & 0.68 & \textbf{0.58} & 0.86 & 0.23 & \textbf{0.66} & 0.41 & 0.58 & 0.39 & \textbf{0.57} & \textbf{0.63} & \textbf{0.58}  \\

%        \hline
%        Ours & 0.71 & 0.72 &0.73 & 0.06 & 0.78 & 0.46 & 0.89 & 0.07 & 0.43 & 0.23 & 0.59 & 0.24 & 0.46 & 0.60 & 0.49\\
%        \hline
%     \end{tabular}
%     \end{adjustbox}
    
%     \label{tab4}
% \end{table*}


% We performed an ablation study to check the efficacy  of architectures without applying probability. We take 1024 X 1024 poster images as input and the output is the multi-hot encoding of the ground truth genres. In Table \ref{tab6} and \ref{tab7}, we present the performance of architectures without probability. We got the best precision
% of 0.95 for animation through our architecture and the best recall
% of 0.99 for drama through  ViT-Dense. Overall our model performed best with the highest micro average,
% macro average precision, and recall respectively 0.60, 0.58,
% 0.64, 0.54. while Res-ViT-Dense was the second-best architecture.

\subsection{Comparison}
In  \autoref{tab:compare}, we present  a comparative
analysis with some major contemporary deep learning architectures such as ResNet50 \cite{he2016deep}, DenseNet121 \cite{8099726}, EfficientNetB2 \cite{tan2019efficientnet}, ViT \cite{dosovitskiy2020image}, InceptionV3  \cite{inceptionv3}, and MobileNetV2 \cite{mobilenetv2}. We have also compared with some important related work \cite{10.1145/3132515.3132516}, and \cite{9057706} and it can also be seen in this table. Our RVD outmatched substantially the vital state-of-the-art methods in terms of $Recall_{macro}$ and $F_1-Measure_{macro}$. Our PrRVD also performed quite well with respect to $Precision_{macro}$ and $Accuracy_{macro}$.


% \subsection{Discussions}


% \textcolor{red}{like Figure-1, we have to check having 1 genre performance?, 2-genre performance?, 3-enre perf?
% xxx
% Utsav: plz write down the discussion informally here that we did now.
% }
% we also have to check genre-wise performance for 1 genre, 2 genre, 3 genre? which are mentioned in figure 1.
% ex- for genre 1,
%     performance for action, comedy, romance etc?
%     for 2 genre - performance for action, comedy, romance etc?



==> old/4resultTable.tex <==
%==================================================
% Table-1
%==================================================

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Performance of proposed RVD and PrRVD over various evaluation metrics}
\label{tab:tab3}
\begin{tabular}{c|c|c}
\hline
\textbf{Metric}& RVD & PrRVD \\
\hline\hline


Macro Precision (${\cal{P}} $) & 0.5501 & \textbf{0.5690} \\
Macro Recall (${\cal{R}} $) & \textbf{0.5725} & 0.5299 \\
Macro F$_1$-Measure (${\cal{FM}} $) & \textbf{0.5569} & 0.5409\\
Macro Accuracy (${\cal{A}} $) & 0.8293 & \textbf{0.8341} \\
Macro Balanced Accuracy (${\cal{BA}} $) & \textbf{0.7216} & 0.7086 \\ 
Macro Specificity (${\cal{S}}p $) & 0.8708 & \textbf{0.8872} \\
Hamming Loss (${\cal{HL}}$) & 0.1707 & \textbf{0.1659} \\ 

\hline
\end{tabular}

\end{table}



% =========================================================
%Table-2
%========================================================
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Performance of various ensembled models}
\label{tab:tab4}
\begin{adjustbox}{width=1\textwidth} 
\begin{tabular}{c |c |c |c |c |c |c |c |c |c |c }
%|c |c |c |c}
\hline
 & \multicolumn{5}{c|}{\textbf{Without Probability}} & \multicolumn{5}{c}{\textbf{With Probability}} \\ \cline{2-11} 
\multirow{-2}{*}{\textbf{Method}} & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{HL}}$ 
%& $\cal{BA}$ & ${\cal{S}}p$ 
& ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{HL}}$ 
%& $\cal{BA}$ & ${\cal{S}}p$ 
\\ \hline \hline

R & 0.5204 & 0.5044 & 0.4897 & 0.8148 & 0.1852 
%& 0.679 & 0.8536
& 0.5456 & 0.4586 & 0.4696 & 0.8216 & 0.1784 
%& 0.6676 & 0.8767
\\

V & 0.2911 & 0.2740 & 0.2258 & 0.7476 & 0.2524 
%& 0.5301 & 0.7861 
& 0.3021 & 0.2174 & 0.1946 & 0.7592 & 0.2408 
%& 0.5248 & 0.8321
\\

RV & 0.5254 & 0.5553 & 0.5357 & 0.8217 & 0.1783 
%& 0.7109 & 0.8667 
& 0.5487 & 0.5272 & 0.5288 & 0.8273 & 0.1727 
%& 0.7039 & 0.8806 
\\

VD & 0.3378 & 0.2981 & 0.2542 & 0.7349 & 0.2651 
%& 0.5448 & 0.7914 
& 0.3020 & 0.2480 & 0.2314 & 0.7499 & 0.2500 
%& 0.5406 & 0.8332 
\\

RVD & 0.5501 & 0.5725 & 0.5569 & 0.8293 & 0.1707 
%& 0.7216 & 0.8708 
& 0.5691 & 0.5299 & 0.5409 & 0.8341 & 0.1659 
%& 0.7086 & 0.8872 
\\

RVD + RV & 0.5496 & \textbf{0.5744} & \textbf{0.5570} & 0.8324 & 0.1676 
%& 0.7236 & 0.8728 
& 0.5740 & \textbf{0.5451} & \textbf{0.5489} & 0.8367 & 0.1633 
%& 0.7156 & 0.8861 
\\

RVD + RV + VD & \textbf{0.5676} & 0.5623 & 0.5514 & \textbf{0.8337} & \textbf{0.1663} 
%& 0.7166 & 0.8708 
& \textbf{0.5907} & 0.5220 & 0.5344 & \textbf{0.8377} & \textbf{0.1623} 
%& 0.7048 & 0.8875 
\\ \hline
 \multicolumn{11}{c}{${\cal{P}} $: Macro Precision, ${\cal{R}} $: Macro Recall, ${\cal{FM}} $: Macro F$_1$-Measure, ${\cal{A}} $: Macro Accuracy, ${\cal{HL}}$: Hamming Loss 
 }%, $\cal{BA}$: Balanced Accuracy, ${\cal{S}}p$: Specificity}
\end{tabular}
\end{adjustbox}
\label{tab:tab2}
\end{table*}


%==================================================
% Table-3
%==================================================
\begin{table}[]
 \centering
 \caption{Comparison of Hit Ratio among various methods.}
 \label{tab:tab5}
 \begin{tabular}{c|c}
 \hline
 \textbf{Method} & Hit Ratio@1 \\
 \hline
 \hline
 R & 0.7224 \\
 V & 0.4626 \\
 RV & 0.7463 \\
 VD & 0.4327 \\
 RVD & 0.7482 \\
 RVD + RV & \textbf{0.7646} \\
 RVD + RV + VD & 0.7558 \\
 \hline
 \end{tabular}
 
\end{table}

%==================================================
% Table-4

%==================================================

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
%  \caption{Gerne-wise performance of RVD.}
%  \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\textbf{Genre}} & \multicolumn{4}{c}{\textbf{Without Probability}} & \multicolumn{4}{c}{\textbf{With Probability}} \\
% \cline{2-9}

%  & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ \\

%  \hline\hline
 
% Action & 0.7603 & 0.6967 & 0.7271 & 0.7748 & 0.7749 & 0.6525 & 0.7084 & 0.7687 \\
% Adventure & 0.7601 & 0.6975 & 0.7275 & 0.8272 & 0.7809 & 0.6749 & 0.7241 & 0.8299 \\
% Animation & 0.8529 & 0.8842 & 0.8683 & 0.9701 & 0.8679 & 0.8415 & 0.8545 & 0.9680 \\
% Biography & 0.2596 & 0.2477 & 0.2535 & 0.8918 & 0.2911 & 0.2110 & 0.2447 & 0.9034 \\
% Comedy & 0.6799 & 0.7476 & 0.7121 & 0.8306 & 0.6839 & 0.7354 & 0.7088 & 0.8306 \\
% Crime & 0.4633 & 0.5359 & 0.4969 & 0.7741 & 0.4771 & 0.5098 & 0.4929 & 0.7816 \\
% Drama & 0.6162 & 0.8523 & 0.7153 & 0.7000 & 0.6244 & 0.8492 & 0.7197 & 0.7075 \\
% Fantasy & 0.3468 & 0.2774 & 0.3082 & 0.8687 & 0.3375 & 0.1742 & 0.2298 & 0.8769 \\
% Horror & 0.5460 & 0.6642 & 0.5993 & 0.8381 & 0.6234 & 0.5373 & 0.5772 & 0.8565 \\
% Mystery & 0.3350 & 0.3131 & 0.3237 & 0.8095 & 0.3579 & 0.2944 & 0.3231 & 0.8204 \\
% Romance & 0.4959 & 0.6316 & 0.5556 & 0.8694 & 0.5000 & 0.6316 & 0.5581 & 0.8707 \\
% Sci-Fi & 0.5455 & 0.3892 & 0.4543 & 0.8823 & 0.5962 & 0.3351 & 0.4291 & 0.8878 \\
% Thriller & 0.4895 & 0.5054 & 0.4973 & 0.7442 & 0.4823 & 0.4429 & 0.4618 & 0.7415 \\
% \hline
% \multicolumn{9}{c}{$\cal{P}$: Precision, $\cal{R}$: Recall, $\cal{FM}$: F$_1$-Measure, $\cal{A}$: Accuracy}
% \end{tabular}
% \end{adjustbox}
% \label{}
% \end{table*}


%==================================================
% Table-4 -Transposed

%==================================================

\begin{table*}[]
\centering
 \caption{Gerne-wise performance of RVD.}
 \label{tab:genre_RVD}
 \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{} & \rotatebox[origin=c]{90}{\textbf{Metric}} & \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller}  \\
\hline
\hline

\multirow{4}{*}{\rotatebox{90}{$W_nProb$}} & ${\cal{P}}_j$ & 0.7603 & 0.7601 & \textbf{0.8529} & 0.2596 & 0.6799 & 0.4633 & 0.6162 & 0.3468 & 0.5460 & 0.3350 & 0.4959 & 0.5455 & 0.4895 \\
 & ${\cal{R}}_j$ & 0.6967 & 0.6975 & \textbf{0.8842} & 0.2477 & 0.7476 & 0.5359 & 0.8523 & 0.2774 & 0.6642 & 0.3131 & 0.6316 & 0.3892 & 0.5054 \\
 & ${\cal{FM}}_j$ & 0.7271 & 0.7275 & \textbf{0.8683} & 0.2535 & 0.7121 & 0.4969 & 0.7153 & 0.3082 & 0.5993 & 0.3237 & 0.5556 & 0.4543 & 0.4973 \\
 & ${\cal{A}}_j$ & 0.7748 & 0.8272 & \textbf{0.9701} & 0.8918 & 0.8306 & 0.7741 & 0.7000 & 0.8687 & 0.8381 & 0.8095 & 0.8694 & 0.8823 & 0.7442 \\

 \hline
\multirow{4}{*}{\rotatebox{90}{$WProb$}} & ${\cal{P}}_j$ & 0.7749 & 0.7809 & \textbf{0.8679} & 0.2911 & 0.6839 & 0.4771 & 0.6244 & 0.3375 & 0.6234 & 0.3579 & 0.5000 & 0.5962 & 0.4823 \\
 & ${\cal{R}}_j$ & 0.6525 & 0.6749 & 0.8415 & 0.2110 & 0.7354 & 0.5098 & \textbf{0.8492} & 0.1742 & 0.5373 & 0.2944 & 0.6316 & 0.3351 & 0.4429 \\
 & ${\cal{FM}}_j$ & 0.7084 & 0.7241 & \textbf{0.8545} & 0.2447 & 0.7088 & 0.4929 & 0.7197 & 0.2298 & 0.5772 & 0.3231 & 0.5581 & 0.4291 & 0.4618 \\
 & ${\cal{A}}_j$ & 0.7687 & 0.8299 & \textbf{0.9680} & 0.9034 & 0.8306 & 0.7816 & 0.7075 & 0.8769 & 0.8565 & 0.8204 & 0.8707 & 0.8878 & 0.7415 \\

 \hline
\multicolumn{15}{c}{$W_nProb$: Without Probability,$WProb$: With Probability, (${\cal{P}}_j$, ${\cal{R}}_j$, ${\cal{FM}}_j$, ${\cal{A}}_j$): Class-wise Precision, Recall, F$_1$-Measure, Accuracy respectively}
\end{tabular}
\end{adjustbox}
\end{table*}

%==================================================
% Table-5

%==================================================

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]

% \centering
%  \caption{Gerne-wise performance of RVD +RV +VD.}
%  \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
%  {\multirow{2}{*}{\textbf{Genre}}} & \multicolumn{4}{c}{\textbf{Without Probability}} & \multicolumn{4}{c}{\textbf{With Probability}} \\
% \cline{2-9}
%  {} & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ \\

% \hline\hline
% Action & 0.7569 & 0.7378 & 0.7472 & 0.7851 & 0.7803 & 0.7014 & 0.7388 & 0.7864 \\
% Adventure & 0.7084 & 0.7449 & 0.7262 & 0.8143 & 0.7298 & 0.7058 & 0.7176 & 0.8163 \\
% Animation & 0.9184 & 0.8232 & 0.8682 & 0.9721 & 0.9241 & 0.8171 & 0.8673 & 0.9721 \\
% Biography & 0.2857 & 0.1284 & 0.1772 & 0.9116 & 0.2647 & 0.0826 & 0.1259 & 0.9149 \\
% Comedy & 0.6513 & 0.7888 & 0.7135 & 0.8224 & 0.6492 & 0.7500 & 0.6959 & 0.8163 \\
% Crime & 0.5246 & 0.5229 & 0.5237 & 0.8021 & 0.5263 & 0.4902 & 0.5076 & 0.8021 \\
% Drama & 0.6039 & 0.8539 & 0.7075 & 0.6878 & 0.6094 & 0.8400 & 0.7063 & 0.6912 \\
% Fantasy & 0.4419 & 0.1226 & 0.1919 & 0.8912 & 0.5172 & 0.0968 & 0.1631 & 0.8952 \\
% Horror & 0.5816 & 0.6119 & 0.5964 & 0.8489 & 0.6515 & 0.4813 & 0.5537 & 0.8585 \\
% Mystery & 0.3779 & 0.3832 & 0.3805 & 0.8184 & 0.3886 & 0.3505 & 0.3686 & 0.8252 \\
% Romance & 0.4936 & 0.6053 & 0.5437 & 0.8687 & 0.4914 & 0.6000 & 0.5403 & 0.8680 \\
% Sci-Fi & 0.5672 & 0.4108 & 0.4765 & 0.8864 & 0.6465 & 0.3459 & 0.4507 & 0.8939 \\
% Thriller & 0.4669 & 0.5761 & 0.5158 & 0.7293 & 0.5000 & 0.5245 & 0.5119 & 0.7497 \\

% \hline
% \multicolumn{9}{c}{$\cal{P}$: Precision, $\cal{R}$: Recall, $\cal{FM}$: F$_1$-Measure, $\cal{A}$: Accuracy}
% \end{tabular}
% \end{adjustbox}
% \label{}
% \end{table*}

%==================================================
% Table-5- Transposed

%==================================================

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
 \caption{Gerne-wise performance of RVD + RV + VD.}
 \label{tab:genre_RVD_RV_VD}
 \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
 \multicolumn{1}{c|}{} & \rotatebox[origin=c]{90}{\textbf{Metric}} & \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} \\

 \hline
 \hline
 
\multirow{4}{*}{\rotatebox{90}{$W_nProb$}} & ${\cal{P}}_j$ & 0.7569 & 0.7084 & \textbf{0.9184} & 0.2857 & 0.6513 & 0.5246 & 0.6039 & 0.4419 & 0.5816 & 0.3779 & 0.4936 & 0.5672 & 0.4669 \\
 & ${\cal{R}}_j$ & 0.7378 & 0.7449 & 0.8232 & 0.1284 & 0.7888 & 0.5229 & \textbf{0.8539} & 0.1226 & 0.6119 & 0.3832 & 0.6053 & 0.4108 & 0.5761 \\
 & ${\cal{FM}}_j$ & 0.7472 & 0.7262 & \textbf{0.8682} & 0.1772 & 0.7135 & 0.5237 & 0.7075 & 0.1919 & 0.5964 & 0.3805 & 0.5437 & 0.4765 & 0.5158 \\
 & ${\cal{A}}_j$ & 0.7851 & 0.8143 & \textbf{0.9721} & 0.9116 & 0.8224 & 0.8021 & 0.6878 & 0.8912 & 0.8489 & 0.8184 & 0.8687 & 0.8864 & 0.7293 \\
 \hline
\multirow{4}{*}{\rotatebox{90}{$WProb$}} & ${\cal{P}}_j$ & 0.7803 & 0.7298 & \textbf{0.9241} & 0.2647 & 0.6492 & 0.5263 & 0.6094 & 0.5172 & 0.6515 & 0.3886 & 0.4914 & 0.6465 & 0.5000 \\
 & ${\cal{R}}_j$ & 0.7014 & 0.7058 & 0.8171 & 0.0826 & 0.7500 & 0.4902 & \textbf{0.8400} & 0.0968 & 0.4813 & 0.3505 & 0.6000 & 0.3459 & 0.5245 \\
 & ${\cal{FM}}_j$ & 0.7388 & 0.7176 & \textbf{0.8673} & 0.1259 & 0.6959 & 0.5076 & 0.7063 & 0.1631 & 0.5537 & 0.3686 & 0.5403 & 0.4507 & 0.5119 \\
 & ${\cal{A}}_j$ & 0.7864 & 0.8163 & \textbf{0.9721} & 0.9149 & 0.8163 & 0.8021 & 0.6912 & 0.8952 & 0.8585 & 0.8252 & 0.8680 & 0.8939 & 0.7497 \\

 \hline
\multicolumn{15}{c}{$W_nProb$: Without Probability,$WProb$: With Probability,
(${\cal{P}}_j$, ${\cal{R}}_j$, ${\cal{FM}}_j$, ${\cal{A}}_j$): Class-wise Precision, Recall, F$_1$-Measure, Accuracy respectively}
%$\cal{P}$: Precision, $\cal{R}$: Recall, $\cal{FM}$: F$_1$-Measure, $\cal{A}$: Accuracy}
\end{tabular}
\end{adjustbox}
\label{}
\end{table*}


%==================================================
% Table-6
%==================================================

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
%  \caption{Gerne-wise performance of RVD + RV.}
%  \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
%  {\multirow{2}{*}{\textbf{Genre}}} & \multicolumn{4}{c}{\textbf{Without Probability}} & \multicolumn{4}{c}{\textbf{With Probability}} \\
%  \cline{2-9}
%  {} & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ & $\cal{P}$ & $\cal{R}$ & $\cal{FM}$ & $\cal{A}$ \\

% \hline
% \hline
 
% Action & 0.7640 & 0.7109 & 0.7365 & 0.7809 & 0.7814 & 0.6888 & 0.7322 & 0.7829 \\
% Adventure & 0.7168 & 0.7551 & 0.7355 & 0.8204 & 0.7282 & 0.7222 & 0.7252 & 0.8191 \\
% Animation & 0.8639 & 0.8902 & 0.8769 & 0.9721 & 0.8781 & 0.8781 & 0.8781 & 0.9728 \\
% Biography & 0.2268 & 0.2018 & 0.2136 & 0.8898 & 0.2338 & 0.1651 & 0.1936 & 0.8979 \\
% Comedy & 0.6722 & 0.7816 & 0.7228 & 0.8319 & 0.6725 & 0.7524 & 0.7102 & 0.8279 \\
% Crime & 0.4927 & 0.5523 & 0.5208 & 0.7884 & 0.4969 & 0.5196 & 0.5079 & 0.7905 \\
% Drama & 0.6283 & 0.8323 & 0.7161 & 0.7082 & 0.6301 & 0.8200 & 0.7126 & 0.7075 \\
% Fantasy & 0.3514 & 0.1677 & 0.2271 & 0.8796 & 0.4565 & 0.1355 & 0.2089 & 0.8918 \\
% Horror & 0.5897 & 0.6008 & 0.5952 & 0.8510 & 0.6542 & 0.5224 & 0.5809 & 0.8626 \\
% Mystery & 0.3632 & 0.3785 & 0.3707 & 0.8129 & 0.3798 & 0.3692 & 0.3744 & 0.8204 \\
% Romance & 0.4878 & 0.6316 & 0.5505 & 0.8667 & 0.4938 & 0.6316 & 0.5543 & 0.8687 \\
% Sci-Fi & 0.4915 & 0.4703 & 0.4807 & 0.8721 & 0.5539 & 0.4162 & 0.4753 & 0.8844 \\
% Thriller & 0.4959 & 0.4946 & 0.4952 & 0.7476 & 0.5029 & 0.4647 & 0.4831 & 0.7510 \\

% \hline
% \multicolumn{9}{c}{$\cal{P}$: Precision, $\cal{R}$: Recall, $\cal{FM}$: F$_1$-Measure, $\cal{A}$: Accuracy}
% \end{tabular}
% \end{adjustbox}
% \label{}
% \end{table*}

%==================================================
% Table-6-Transposed
%==================================================

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
 \caption{Gerne-wise performance of RVD + RV.}
 \label{tab:genre_RVD_RV}
 \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
 \multicolumn{1}{c|}{} & \rotatebox[origin=c]{90}{\textbf{Metric}} & \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} \\

 \hline
 \hline
\multirow{4}{*}{\rotatebox{90}{$W_nProb$}} & ${\cal{P}}_j$ & 0.7640 & 0.7168 & \textbf{0.8639} & 0.2268 & 0.6722 & 0.4927 & 0.6283 & 0.3514 & 0.5897 & 0.3632 & 0.4878 & 0.4915 & 0.4959 \\
 & ${\cal{R}}_j$ & 0.7109 & 0.7551 & \textbf{0.8902} & 0.2018 & 0.7816 & 0.5523 & 0.8323 & 0.1677 & 0.6008 & 0.3785 & 0.6316 & 0.4703 & 0.4946 \\
 & ${\cal{FM}}_j$ & 0.7365 & 0.7355 & \textbf{0.8769} & 0.2136 & 0.7228 & 0.5208 & 0.7161 & 0.2271 & 0.5952 & 0.3707 & 0.5505 & 0.4807 & 0.4952 \\
 & ${\cal{A}}_j$ & 0.7809 & 0.8204 & \textbf{0.9721} & 0.8898 & 0.8319 & 0.7884 & 0.7082 & 0.8796 & 0.8510 & 0.8129 & 0.8667 & 0.8721 & 0.7476 \\
 \hline
\multirow{4}{*}{\rotatebox{90}{$WProb$}} & ${\cal{P}}_j$ & 0.7814 & 0.7282 & \textbf{0.8781} & 0.2338 & 0.6725 & 0.4969 & 0.6301 & 0.4565 & 0.6542 & 0.3798 & 0.4938 & 0.5539 & 0.5029 \\
 & ${\cal{R}}_j$ & 0.6888 & 0.7222 & \textbf{0.8781} & 0.1651 & 0.7524 & 0.5196 & 0.8200 & 0.1355 & 0.5224 & 0.3692 & 0.6316 & 0.4162 & 0.4647 \\
 & ${\cal{FM}}_j$ & 0.7322 & 0.7252 & \textbf{0.8781} & 0.1936 & 0.7102 & 0.5079 & 0.7126 & 0.2089 & 0.5809 & 0.3744 & 0.5543 & 0.4753 & 0.4831 \\
 & ${\cal{A}}_j$ & 0.7829 & 0.8191 & \textbf{0.9728} & 0.8979 & 0.8279 & 0.7905 & 0.7075 & 0.8918 & 0.8626 & 0.8204 & 0.8687 & 0.8844 & 0.7510 \\

  \hline
\multicolumn{15}{c}{$W_nProb$: Without Probability,$WProb$: With Probability, 
(${\cal{P}}_j$, ${\cal{R}}_j$, ${\cal{FM}}_j$, ${\cal{A}}_j$): Class-wise Precision, Recall, F$_1$-Measure, Accuracy respectively}
%$\cal{P}$: Precision, $\cal{R}$: Recall, $\cal{FM}$: F$_1$-Measure, $\cal{A}$: Accuracy}
\end{tabular}
\end{adjustbox}
\label{}
\end{table*}


%==================================================
% Table-8
%==================================================
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
 \caption{Performance comparison with respect to number of genre labels}
 \label{tab:genre_ALL}
 \begin{adjustbox}{width=1\textwidth} 
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
 & & \multicolumn{4}{c|}{ \textbf{1 Genre}} & \multicolumn{4}{c|}{ \textbf{2 Genre}} & \multicolumn{4}{c}{\textbf{3 Genre}} \\
 \cline{3-14}

 
\multirow{-2}{*}{ \textbf{}} & \multirow{-2}{*}{ \textbf{Method}} & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ \\

\hline
\hline

 & RVD & 0.0957 & 0.2094 & 0.1043 & 0.8112 & 0.3890 & \textbf{0.5517} & \textbf{0.4337} & 0.8244 & 0.5648 & 0.5623 & \textbf{0.5588} & 0.8305 \\
 & RVD+RV & 0.0938 & 0.1838 & 0.1063 & \textbf{0.8252} & 0.3805 & 0.5425 & 0.4218 & 0.8271 & 0.5657 & \textbf{0.5628} & 0.5586 & 0.8336 \\
\multirow{-3}{*}{\textbf{Without Probability}} & RVD+RV+VD & \textbf{0.0959} & \textbf{0.2180} & \textbf{0.1091} & \textbf{0.8252} & \textbf{0.3906} & 0.5285 & 0.4194 & \textbf{0.8291} & \textbf{0.5814} & 0.5505 & 0.5519 & \textbf{0.8347} \\
\hline

 & RVD & 0.0951 & 0.1923 & 0.0936 & 0.8252 & 0.3994 & 0.4719 & 0.4045 & 0.8325 & 0.5822 & 0.5229 & 0.5434 & 0.8346 \\
 & RVD+RV & 0.0935 & 0.1667 & 0.0972 & 0.8252 & 0.3941 & \textbf{0.5168} & \textbf{0.4192} & 0.8353 & 0.5876 & \textbf{0.5331} & \textbf{0.5494} & 0.8372 \\
 
\multirow{-3}{*}{\textbf{With Probability}} & RVD+RV+VD & \textbf{0.0967} & \textbf{0.1966} & \textbf{0.0987} & \textbf{0.8322} & \textbf{0.4050} & 0.4801 & 0.4018 & \textbf{0.8370} & \textbf{0.6038} & 0.5120 & 0.5352 & \textbf{0.8379} \\
\hline

\multicolumn{14}{c}{${\cal{P}} $: Macro Precision, ${\cal{R}} $: Macro Recall, ${\cal{FM}} $: Macro F$_1$-Measure, ${\cal{A}} $: Macro Accuracy,} 
%${\cal{HL}}$: Hamming Loss , $\cal{BA}$: Balanced Accuracy, ${\cal{S}}p$: Specificity}
\end{tabular}
\end{adjustbox}
\label{}
\end{table*}



%==================================================
% Table-7
%==================================================

\begin{table}[]
\centering
\caption{Comparison Among various baseline methods.}
\label{tab:compare}
\begin{tabular}{c|c|c|c|c}
\hline
 \textbf{Method} & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ \\
 \hline
 \hline
ResNet50 \cite{he2016deep} & 0.5204 & 0.5044 & 0.4897 & 0.8148 \\
DenseNet121 \cite{8099726}  & 0.2610 & 0.2718 & 0.2263 & 0.6988 \\
EfficientNetB2  \cite{tan2019efficientnet} & 0.5137 & 0.5253 & 0.5140 & 0.8150 \\
ViT \cite{dosovitskiy2020image} & 0.2911 & 0.2740 & 0.2258 & 0.7476 \\
InceptionV3 \cite{inceptionv3} & 0.2103 & 0.2879 & 0.2243 & 0.7440 \\
MobileNetV2 \cite{mobilenetv2} & 0.3734 & 0.3322 & 0.3037 & 0.7620 \\
\hline
Chu et al. \cite{10.1145/3132515.3132516} & 0.1973 & 0.2732 & 0.2089 & 0.6896\\
Wi et al. \cite{9057706} & 0.5289 & 0.5118 & 0.4961 & 0.8282\\
\textbf{RVD (Ours)} & 0.5501 & \textbf{0.5725} & \textbf{0.5569} & 0.8293 \\
\textbf{PrRVD (Ours)} & \textbf{0.5690} & 0.5299 & 0.5409 & \textbf{0.8341}\\
\hline

\multicolumn{5}{c}{${\cal{P}} $: Macro Precision, ${\cal{R}} $: Macro Recall,} \\
\multicolumn{5}{c}{${\cal{FM}} $: Macro F$_1$-Measure, ${\cal{A}} $: Macro Accuracy}


\end{tabular}
\end{table}
% %==================================================
% % Table-8
% %==================================================
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \centering
%  \caption{Performance comparison with respect to number of genre labels}
%  \begin{adjustbox}{width=1\textwidth} 
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
%  & & \multicolumn{4}{c|}{ \textbf{1 Genre}} & \multicolumn{4}{c|}{ \textbf{2 Genre}} & \multicolumn{4}{c}{\textbf{3 Genre}} \\
%  \cline{3-14}

 
% \multirow{-2}{*}{ \textbf{}} & \multirow{-2}{*}{ \textbf{Method}} & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ & ${\cal{P}} $ & ${\cal{R}} $ & ${\cal{FM}} $ & ${\cal{A}} $ \\

% \hline
% \hline

%  & RVD & 0.0957 & 0.2094 & 0.1043 & 0.8112 & 0.3890 & 0.5517 & 0.4337 & 0.8244 & 0.5648 & 0.5623 & 0.5588 & 0.8305 \\
%  & RVD+RV & 0.0938 & 0.1838 & 0.1063 & 0.8252 & 0.3805 & 0.5425 & 0.4218 & 0.8271 & 0.5657 & 0.5628 & 0.5586 & 0.8336 \\
% \multirow{-3}{*}{\textbf{Without Probability}} & RVD+RV+VD & 0.0959 & 0.2180 & 0.1091 & 0.8252 & 0.3906 & 0.5285 & 0.4194 & 0.8291 & 0.5814 & 0.5505 & 0.5519 & 0.8347 \\
% \hline

%  & RVD & 0.0951 & 0.1923 & 0.0936 & 0.8252 & 0.3994 & 0.4719 & 0.4045 & 0.8325 & 0.5822 & 0.5229 & 0.5434 & 0.8346 \\
%  & RVD+RV & 0.0935 & 0.1667 & 0.0972 & 0.8252 & 0.3941 & 0.5168 & 0.4192 & 0.8353 & 0.5876 & 0.5331 & 0.5494 & 0.8372 \\
 
% \multirow{-3}{*}{\textbf{With Probability}} & RVD+RV+VD & 0.0967 & 0.1966 & 0.0987 & 0.8322 & 0.4050 & 0.4801 & 0.4018 & 0.8370 & 0.6038 & 0.5120 & 0.5352 & 0.8379 \\
% \hline

% \multicolumn{14}{c}{${\cal{P}} $: Precision, ${\cal{R}} $: Recall, ${\cal{FM}} $: F$_1$-Measure, ${\cal{A}} $: Accuracy}
% \end{tabular}
% \end{adjustbox}
% \label{}
% \end{table*}

%==================================================
% Table-x

%==================================================
% Table-x

%==================================================
% Table-x

%==================================================
% Table-x

%==================================================

==> old/others.tex <==

\begin{table*}[]
    \centering
    \begin{tabular}{c|c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
      \hline \backslashbox{Methods}{Genres}  & Evaluation Matrix &  \rotatebox[origin=c]{90}{Action} & \rotatebox[origin=c]{90}{Adventure} & \rotatebox[origin=c]{90}{Animation} & \rotatebox[origin=c]{90}{Biography} & \rotatebox[origin=c]{90}{Comedy} & \rotatebox[origin=c]{90}{Crime} & \rotatebox[origin=c]{90}{Drama} & \rotatebox[origin=c]{90}{Fantasy} & \rotatebox[origin=c]{90}{Horror} & \rotatebox[origin=c]{90}{Mystery} & \rotatebox[origin=c]{90}{Romance} & \rotatebox[origin=c]{90}{Sci-Fi} & \rotatebox[origin=c]{90}{Thriller} \\
      \hline \hline
       ResNet50  & Precision \\\cline{2-3}
         & Recall \\
         \hline
       DenseNet121  & Precision \\\cline{2-3}
         & Recall \\
       \hline
       EfficientNetB2  & Precision \\\cline{2-3}
         & Recall \\
         \hline
       ViT  & Precision \\\cline{2-3}
       & Recall \\
       \hline
       Ensemble & Precision \\\cline{2-3}
         & Recall \\
       \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}






\begin{table*}
\begin{center}
\caption{Precision comparison of Top 3 genres without probability.}
\label{tab2}
\begin{tabular}{ l | c | c | c | c | c | c | c | c }
\hline \backslashbox{Genres}{Methods} & ResNet50 & DenseNet121 & EfficientNetB2 & ViT & Res-ViT & ViT-Dense & Res-ViT-Dense & Ensemble\\ \hline \hline
Action & 0.66 & 0.36 & 0.70 & 0.47 & 0.75 & 0.46 & 0.76 & 0.72 \\
\hline
Adventure & 0.66 & 0.50 & 0.73 & 0.37 & 0.67 & 0.44 & 0.82 & 0.7\\
\hline
Animation & 0.87 & 0.17 & 0.84 & 0 & 0.87 & 0.43 & 0.86 & 0.95\\
\hline
Biography & 0.21 & 0.05 & 0.24 & 0 & 0.18 & 0 & 0.27 & 0.34\\
\hline
Comedy & 0.60 & 0.47 & 0.62 & 0.46 & 0.66 & 0.32 & 0.74  & 0.63\\
\hline
Crime & 0.46 & 0.5 & 0.43 & 0.29 & 0.46 & 0.29 & 0.43 & 0.52\\
\hline
Drama & 0.57 & 0.49 & 0.60 & 0.45 & 0.63 & 0.44 & 0.6 & 0.57\\
\hline
Fantasy & 0.36 & 0 & 0.24 & 0.18 & 0.29 & 0 & 0.36 & 0.52\\
\hline
Horror & 0.50 & 0.3 & 0.54 & 0.35 & 0.59 & 0.29 & 0.54 & 0.55\\
\hline
Mystery & 0.41 & 0 & 0.31 & 0.3 & 0.36 & 0.15 & 0.37 & 0.38\\
\hline
Romance & 0.48 & 0.12 & 0.48 & 0.33 & 0.45 & 0.21 & 0.52 & 0.54\\
\hline
Sci-Fi & 0.56 & 0.2 & 0.48 & 0.25 & 0.44 & 0.3 & 0.55 & 0.61\\
\hline
Thriller & 0.43 & 0.24 & 0.46 & 0.34 & 0.46 & 0.4 &  0.47 & 0.47\\
\hline
\end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Recall comparison of Top 3 genres without probability.}
\label{tab3}
\begin{tabular}{ l | c | c | c | c | c | c | c | c }
\hline \backslashbox{Genres}{Methods} & ResNet50 & DenseNet121 & EfficientNetB2 & ViT & Res-ViT & ViT-Dense & Res-ViT-Dense & Ensemble\\ \hline \hline 
Action & 0.73 & 0.16 & 0.74 & 0.8 & 0.68 & 0.74 & 0.67 & 0.77 \\
\hline
Adventure & 0.67 & 0.1 & 0.68 & 0.72 & 0.75 & 0.08 & 0.62  & 0.76\\
\hline
Animation & 0.80 & 0.09 & 0.82 & 0 & 0.87 & 0.16 & 0.87 & 0.74 \\
\hline
Biography & 0.04 & 0.07 & 0.11 & 0 & 0.17 & 0 & 0.37 & 0.09\\
\hline
Comedy & 0.75 & 0.77 & 0.69 & 0.53 & 0.76  & 0.92 & 0.68  & 0.8\\
\hline
Crime & 0.45 & 0.01 & 0.57 & 0.06 & 0.52 & 0.03 & 0.58 & 0.49\\
\hline
Drama & 0.88 & 0.93 & 0.81 & 0.98 & 0.78 & 0.99 & 0.86 & 0.9\\
\hline
Fantasy & 0.05 & 0 & 0.25 & 0.06 & 0.14 & 0 & 0.23 & 0.08\\
\hline
Horror & 0.53 & 0.34 & 0.52 & 0.21 & 0.54 & 0.26 & 0.66 & 0.56\\
\hline
Mystery & 0.26 & 0 & 0.33 & 0.03 & 0.43 & 0.03 & 0.41 & 0.3\\
\hline
Romance & 0.58 & 0.79 & 0.56 & 0.01 & 0.61 & 0.3 & 0.58 & 0.59\\
\hline
Sci-Fi & 0.29 & 0.24 & 0.32 & 0.01 & 0.52 & 0.02 & 0.39 & 0.29\\
\hline
Thriller & 0.54 & 0.03 & 0.45 & 0.14 & 0.45 & 0.02  &  0.57 & 0.57\\
\hline

\end{tabular}
\end{center}
\end{table*}


==> tables/1relatedTable.tex <==



\begin{table*}[!htb]
    \centering
    \caption{Summary of Related Work}% without probability
   \begin{adjustbox}{width=1\textwidth} 
    \begin{tabular}{c | c | c | c | c | c | c| c}
   % \cline{2-8} 
   \hline
      &  Method & Year & Input & Architecture/ Technique & \# Genre/\#Tags & Dataset & Multi-label?\\
      \hline \hline
\multirow{6}{*}{\rotatebox{90}{Textual}} & Mukta et al. \cite{Mukta_Khan_Ali_Mahmud_2017} & 2017 & Tweets  & Na\"ive Bayes, SVM, Random Forest, & 5 &  IMDb, Twitter (Pvt.) & $\upchi$\\ \cline{2-8} 
       & Ertugrul et al. \cite{ertugrul2018movie} & 2018 & Synopsis & BLSTM based & 4 & Pvt. & $\upchi$\\ \cline{2-8}
       & Hoang et al. \cite{hoang2018predicting} & 2018 & Synopsis &  Naive Bayes, XGBoost, GRU & 20 & IMDb (Pvt.) & \checkmark\\ \cline{2-8}
       & Kar et al. \cite{kar-etal-2018-folksonomication} & 2018 & Synopsis & CNN, BLSTM& 71 & MPST  & \checkmark\\ \cline{2-8}
       & Battu et al. \cite{battu-etal-2018-predicting} & 2018 & Synopsis & CNN, LSTM-based & 9 & MLMRD  & $\upchi$\\ \cline{2-8}
       
       & Wehrmann et al. \cite{wehrmann2018self} & 2018 & Synopsis & Self-Attention & 9 & LMTD-9 & \checkmark \\
       \cline{2-8}
       & Portolese et al. \cite{portolese2018use} & 2018 & Synopsis & Desicion Tree, MLP & 12 & TMDb (Pvt.) & \checkmark\\
       \cline{2-8}
       & Portolese et al. \cite{portolese2019exploring} & 2019 & Synopsis & Binary Relevance, RAKEL & 18 & P-TMDb (Pvt.) & \checkmark\\
       & & & & Classifier Chains, DBPNN& & \\
       \cline{2-8}
       & Saputra et al. \cite{saputra2019classification} & 2019 & Synopsis & Naive Bayes, SVM, MLP & 5 & IMDb (Pvt.) & $\upchi$\\ \cline{2-8}
       & Gorinski et al. \cite{gorinski-lapata-2018-whats} & 2018 & Screenplay & LSTM-based decoder & 31 & Pvt. & \checkmark\\ \cline{2-8}
       %& Lee et al. \cite{lee2002text} & 2002 & Text & Na\"ive Bayes Classiﬁer & 7 & Pvt.  &  \\ \cline{2-8}
       %& Stamatatos et al. \cite{stamatatos2000automatic}   & 2000 & Text & Discriminant Analysis,   & 10 & Pvt.  &  \\ \cline{2-8}
       % &   Kessler et al. \cite{kessler-etal-1997-automatic}   & 1997 & Text & Linear Regression & 6 & Pvt.   & \\ \cline{2-8}
     %  &  Biber et al. \cite{biber1986spoken}  & 1986 & Text &  &  &  &  \\ \cline{2-8}
     %  &    &  &  &  &  &   & \\ \cline{2-8}
       % &    &  &  &  &  &   & \\ \cline{2-8}
%=============================
\hline
  % & Fischer et al. \cite{10.1145/217279.215283} & 1995 & Video & Content Processing (CoP) Algorithm & 5 & Pvt. & \\
\multirow{12}{*}{\rotatebox{90}{Visual}} 
& Rasheed et al \cite{1377360} & 2005 & Trailer & Mean Shift Classification & 4 & Pvt. & \checkmark \\
\cline{2-8}
    & Huang et al. \cite{4412917} & 2007 & Trailer & Decision Tree & 3 & Pvt. & $\upchi$\\ 
    \cline{2-8}
    %Avg. Shot Length, Color Variance & & & \\
    %& & & & Motion Content, Lighting Key & & & \\\cline{2-8}

& Zhou et al. \cite{zhou2010movie} & 2010 & Trailer & K-means, KNN, GIST, & 4 & Pvt.  & $\upchi$ \\ 
& & & & CENTRIST, W-CENTRIST & & & \\
\cline{2-8}
% & Truong et al. \cite{truong2000automatic}  & 2000 & Video & Decision Tree & 5 & Pvt. & \\ \cline{2-8} 
    & Yuan et al. \cite{4107177} & 2006  & Trailer & SVM Binary Tree &  4 & Pvt. & $\upchi$\\ \cline{2-8} 
    % & Sande et al. \cite{5204091} & 2010 &        
    & Huang et al. \cite{huang2012movie} & 2012 & Trailer & SAHS, SVM & 7 & AMT, IMDb (Pvt.) & $\upchi$\\ \cline{2-8}
    & Simoes et al.  \cite{Simes2016MovieGC} & 2016 & Trailer & CNN-MoTion & 4 & LMTD-4 & $\upchi$ \\ \cline{2-8}
    & Wehrmann et al.\cite{wehrmann2017movie} \cite{10.1145/3019612.3019641} & 2017 & Trailer & CTT-MMC & 9 & LMTD-9 & \checkmark \\ \cline{2-8}
     & Lezama et al. \cite{montalvo2022trailers12k} & 2022 & Trailer &  Transformer & 10 & Trailers12k  & \checkmark\\ \cline{2-8}
     
    & Ashima at al. \cite{yadav2020unified} & 2020 & Facial Frame & Inception-LSTM & 6 & EmoGDB (Pvt.)  &  \checkmark \\ \cline{2-8}
   
    %& Ghaemmaghami et al. \cite{ghaemmaghami2015movie} & 2015 & MEG Signal & Naive Bayes Classiﬁer & 4 & Pvt. & $\upchi$\\ \cline{2-8}
    
    & Ivasic-Kos et al. 
    %\cite{ivasic2014movie}, \cite{ivasic2015automatic}, 
    \cite{pobar2017multi} & 2017 & Poster & Naive Bayes, RAKEL, binary relevance & %6,18,
    18 & TMDb (Pvt.) & \checkmark \\ 
    \cline{2-8}
    & Chu et al. \cite{10.1145/3132515.3132516} & 2017 & Poster & CNN, YOLO & 23 & IMDb (Pvt.)  &  \checkmark\\ \cline{2-8}
    & Gozuacik et al. \cite{8990490} & 2019 & Poster & CNN & 4 & Pvt. & $\upchi$ \\ \cline{2-8}
    & Wi et al. \cite{9057706} & 2020 & Poster & CNN, Gram layer & 12 & IMDb (Pvt.) &  \checkmark\\ \cline{2-8}
    & \textbf{Ours}   & - & Poster & Transformer & 13 & IMDb & \checkmark \\ \cline{2-8}
    & Ghaemmaghami et al. \cite{ghaemmaghami2015movie} & 2015 & MEG Signal & Naive Bayes Classiﬁer & 4 & Pvt. & $\upchi$\\ \cline{2-8}
%=============================
\hline
\multirow{7}{*}{\rotatebox{90}{Multimodal}}
    & Rasheed et al. \cite{1048494} & 2002 & Trailer, Audio & Linear Classifier, Visual disturbance & 4 & Pvt. & $\upchi$\\
    & & & & Avg. Shot Length, Audio Energy & & & \\ \cline{2-8}
    
    & Brezeale et al. \cite{brezeale2006using} & 2006 & Video, Subtitle & SVM, DCT, Bag-of-Word & 18 & Pvt. & \\ \cline{2-8} 
%    & Rouvier et al. \cite{rouvier2015audio} & 2015 &  Video, Audio, Text & SVM, ANN & 7 & Pvt. & $\upchi$\\ \cline{2-8}
    & Huang et al. \cite{huang2020movienet} & 2020 & Scene image, Trailer & ResNet50, TRN\cite{zhou2018temporal} & 21 & MovieNet & \checkmark\\ \cline{2-8}    
    & Bonilla et al. \cite{cascante2019moviescope} & 2019 & Poster, Video, Audio, Synopsis, Metadata & VGG-19, RCNN, LSTM & 13 & Moviescope  & \checkmark\\ 
    & & & & fastText, fastVideo & & & \\\cline{2-8}
  %     & Ekenel et al. \cite{ekenel2013multimodal} & 2013 & Video, Audio, Metadata & SVM & 7 & Pvt. & -\\ \cline{2-8}
       & Mangolin et al. \cite{mangolin2022multimodal} & 2022 & trailers, subtitle, synopses, poster & Textural feature, LSTM, CNN & 18 & TMDb (Pvt.) & \checkmark \\
       \cline{2-8}

       & Arevalo et al. \cite{arevalo2017gated} & 2017 & Poster, Synopsis, metadata & Word2Vec, CNN-based, GMU & 23 & MM-IMDb & \checkmark \\ 
       \cline{2-8}
       & Bribiesca et al. \cite{bribiesca2021multimodal} & 2021 & Poster, Video, Audio, Synopsis, Metadata & Transformer, GMU & 13 & Moviescope & \checkmark \\ 
       \cline{2-8}

       & Hong et al. \cite{hong2015multimodal} & 2015 & Video, Audio, Text & Probabilistic Latent Semantic Analysis & 4 & IMDb, Douban (Pvt.) & $\upchi$ \\
       \cline{2-8}

       & Fu et al. \cite{fu2015fast} & 2015 & Poster, Synopsis & SVM & 4 & TMDb (Pvt.) & $\upchi$ \\
       \hline


% \textbf{BLSTM}: Bidirectional Long Short-Term Memory,
%     \textbf{XGBoost}: Extreme Gradient Boosting, 
%     \textbf{GRU}: Gated Recurrent Units, 
%     \textbf{CNN}: Convolutional Neural Network,
%     \textbf{LSTM}: Long Short-Term Memory,
%     \textbf{KNN}: K-Nearest Neighbor,
%     \textbf{SVM}: Support Vector Machine, 
%     \textbf{CNN-Motion}: CNN for Movie Trailer Classification,
%        \textbf{CTT-MMC}: Convolution Through Time for Multi-label Movie genre Classification
%        \textbf{YOLO}: You Only Look Once,
%        \textbf{ANN}: Artificial Neural Network,
%        \textbf{TRN}: Temporal Relation Network 
%        \textbf{RCNN}: Region-Based CNN
%         \textbf{MLP}: Multi-Layer Perceptron
%         \textbf{RAKEL}: Random k-Labelset
%         \textbf{DBPNN}: Deep Back-Propagation Neural Network
%         \textbf{SAHS}:  Self-Adaptive Harmony Search
%         \textbf{DCT}:  Discrete Cosine Transform
%         \textbf{GMU}:  Gated Multimodal Unit


        
       % \textbf{IMDb}: Internet Movie Database,
       % \textbf{MPST}: Movie Plot Synopses with Tags 
       % \textbf{MLMRD}: Multi-Language Movie Review Dataset
       % \textbf{LMTD}: Labeled Movie Trailer Data
       % 
       % \textbf{EmoGDB}: Emotional-based Genre Detection for Bollywood
       % \textbf{MMTF-14K}: Multifaceted Movie Trailer Feature-14K
       % \textbf{ML-25M}: MovieLens-25M
       % \textbf{TMDb}: The Movie Database 
      % \textbf{AMT}: Apple iTunes Movie Trailers
         % \textbf{MM-IMDb}: Multimodal IMDb
       
    \end{tabular}
    \end{adjustbox}
    
    \label{tab:related_work}
\end{table*}





%text/meta data/ sub-title 
% Over the years, Researchers have worked on the automatic genre classification problem and proposed various methods. 
% https://dl.acm.org/doi/abs/10.1145/3459637.3482018
% https://arxiv.org/abs/2211.05044
% https://arxiv.org/abs/1801.04813
% https://dl.acm.org/doi/10.1145/564376.564403
% https://ieeexplore.ieee.org/abstract/document/9453021
% https://dl.acm.org/doi/abs/10.1145/3449103
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=5495763&tag=1



%These datasets are publicly unavailable at time of our research work, Therefore we construct new dataset and processed on it.
%our: only poster, no textual info

%textual
% https://www.jstor.org/stable/414678
%https://aclanthology.org/P97-1005/
% https://direct.mit.edu/coli/article/26/4/471/1675/Automatic-Text-Categorization-in-Terms-of-Genre
% https://aclanthology.org/C00-2117.pdf
% https://aclanthology.org/N18-1160/

% https://aclanthology.org/Y18-1007.pdf

% https://aclanthology.org/L18-1274.pdf
% https://aclanthology.org/C18-1244.pdf
% https://dl.acm.org/doi/abs/10.1145/3442381.3449806

% https://dblp.org/pid/189/4618.html
% https://openaccess.thecvf.com/content/CVPR2021W/CVFAD/html/Agrawal_Color_Me_Good_Branding_in_the_Coloring_Style_of_Movie_CVPRW_2021_paper.html


% dataset
%https://link.springer.com/chapter/10.1007/978-3-030-58548-8_41

% hybrid
% https://arxiv.org/abs/1908.03180
% https://link.springer.com/article/10.1007/s11042-020-10086-2

%videos/visual

% https://www.researchgate.net/publication/3421929_Automatic_Video_Classification_A_Survey_of_the_Literature

% https://dl.acm.org/doi/10.1145/217279.215283

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=902901
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7727207
% https://dl.acm.org/doi/abs/10.1145/1873951.1874068?casa_token=Lybn5suT-qYAAAAA:zoY6Rzf3OsbEHlZmv3eQh9x2HtslKyAHn_3FGy3tCbs0tGzPV4AC0IQj-3WusoS07N7GUmangt4UBw

% https://www.sciencedirect.com/science/article/pii/S1568494620305627
% https://www.sciencedirect.com/science/article/pii/S1568494617305112

%https://dl.acm.org/doi/abs/10.1145/3019612.3019641?casa_token=VfEjBCN6eU8AAAAA:fdXGddB3g9MJvn-un6pvDpaP8i_4yI9vQ2V-VtoE0y-Jh3cJYOyyZNu8VuEI0Y9H9ZTX-1Z074cpyg
%https://ieeexplore.ieee.org/abstract/document/7965908
% https://link.springer.com/chapter/10.1007/978-3-031-25069-9_42

% https://ieeexplore.ieee.org/abstract/document/9412480
%http://cs230.stanford.edu/projects_winter_2020/reports/32643471.pdf
%http://cs230.stanford.edu/projects_fall_2021/reports/102983714.pdf
% https://ieeexplore.ieee.org/abstract/document/902901
% https://ieeexplore.ieee.org/abstract/document/4107177
% % https://ieeexplore.ieee.org/abstract/document/6977171
% https://ieeexplore.ieee.org/document/5495042

% posters
% https://dl.acm.org/doi/abs/10.1145/3132515.3132516?casa_token=rFWpLC_aCKgAAAAA:VwkvnqQUXw7mjL0cFvhNM_uSweRYKjF090nmSe8bjEt4BIz8tczGUx8ZsYrnuLpR4osrOUo7vX-a5w
% https://ieeexplore.ieee.org/abstract/document/9506751
% https://link.springer.com/chapter/10.1007/978-3-319-23231-7_61
%https://ieeexplore.ieee.org/abstract/document/8990490
% https://link.springer.com/article/10.1007/s11042-011-0923-x
%https://link.springer.com/article/10.1007/s11042-020-10086-2
%others




%https://ieeexplore.ieee.org/abstract/document/9276019
%https://ieeexplore.ieee.org/abstract/document/9453021
% https://ieeexplore.ieee.org/abstract/document/9276019
% https://dl.acm.org/doi/abs/10.1145/3132515.3132516?casa_token=msjcCFGyz9MAAAAA:O314n59rEb5ntPtjDXzbRDuDMMLygJa6c8asMwbmfUVkggUXSZUmD45rYHSVBdt0QDzCvHeGxrwYOQ

% https://dl.acm.org/doi/abs/10.1145/3348445.3348475

% https://link.springer.com/article/10.1007/s11042-020-10125-y
% 
% 
% % https://ieeexplore.ieee.org/abstract/document/9190344
% 


% transactions
% https://ieeexplore.ieee.org/abstract/document/6071010
% % https://ieeexplore.ieee.org/document/7001198
% https://ieeexplore.ieee.org/abstract/document/1377360
% % https://ieeexplore.ieee.org/abstract/document/5204091

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6471714

%into
% Howard, I. P., & Templeton, W. B. Human spatial orientation. New York: Wiley, 1966
% Visual Dominance: An Information-Processing Account of Its Origins and Significance
% A sensorimotor account of vision and visual consciousness




% new July
%not
% Sugano, M., Isaksson, R., Nakajima, Y., Yanagihara, H.: Shot genre classification using compressed audio-visual features. In: International Conference on Image Processing (2003)

% Huang, H.Y., Shih, W.S., Hsu, W.H.: A film classifier based on low-level visual features. In: IEEE Workshop on Multimedia Signal Processing. pp. 465–468 (2007

%not
% Nam, J., Alghoniemy, M., Tewfik, A.H.: Audio-visual content-based violent scene characterization. In: International Conference on Image Processing

% Isaac Rodr´ıguez Bribiesca, Adrian Pastor L ´ opez Monroy, and Manuel Montes-y ´ Gomez. Multimodal weighted fusion of Transformers for movie genre classification. In Proceedings of the Third Workshop on Multimodal Artificial Intelligence, pages 1–5, Mexico City, Mexico, June 2021. Association for Computational Linguistics. doi: 10.18653/v1/2021.maiworkshop-1.1.

% Yin-Fu Huang and Shih-Hao Wang. Movie genre classification using SVM with audio and video features. In International Conference on Active Media Technology, pages 1–10. Springer, 2012

% Marina Ivasic-Kos, Miran Pobar, and Luka Mikec. 2014. Movie Posters Classification into Genres based on Low-level Features. In Proceedings of International Convention on Information and Communication Technology, Electronics and Microelectronics

% Marina Ivasic-Kos, Miran Pobar, and Luka Mikec. 2014. Automatic Movie Posters Classification into Genres. In Proceedings of ICT Innovation. 319–328


%v M. Pobar and M. Ivasic-Kos, “Multi-label poster classiﬁcation into gen-res using different problem transformation methods,” in InternationalConference on Computer Analysis of Images and Patterns. Springer,2017, pp. 367–378


% J. Wehrmann, M. A. Lopes, and R. C. Barros, “Self-attention forsynopsis-based multi-label movie genre classiﬁcation,” in The Thirty-FirstInternational Flairs Conference, 2018

% A. C. Saputra, A. B. Sitepu, P. W. Y. Sigit, P. G. S. A. Tetuko, G. C.Nugroho et al., “The classiﬁcation of the movie genre based on synopsisof the indonesian ﬁlm,” in 2019 International Conference of ArtiﬁcialIntelligence and Information Technology (ICAIIT). IEEE, 2019, pp. 201–20


% Huang, Q., Xiong, Y., Xiong, Y., Zhang, Y., Lin, D.: From trailers to storylines: An efficient way to learn from movies. arXiv preprint arXiv:1806.05341 (2018) 9

% M. Tapaswi, M. Bauml, and R. Stiefelhagen. Book2movie: Aligning video scenes with book chapters. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, pages 1827–1835, 2015

% Y. Zhu, R. Kiros, R. Zemel, R. Salakhutdinov, R. Urtasun, A. Torralba, and S. Fidler. Aligning books and movies: Towards story-like visual explanations by watching movies and reading books. In Proceedings of the IEEE international conference on computer vision, pages 19–27, 2015.

% M. Tapaswi, Y. Zhu, R. Stiefelhagen, A. Torralba, R. Urtasun, and S. Fidler. Movieqa: Understanding stories in movies through question-answering. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, pages 4631–4640, 2016

% Hong H-Z, Hwang J-IG (2015) Multimodal PLSA for movie genre classification. In: Proceedings of the International workshop on multiple classifier systems. Springer, pp 159–167

% Huang Y-F, Wang S-H (2012) Movie genre classification using svm with audio and video features. In: Proceedings of the International conference on active media technology. Springer, pp 1–10

% Fu Z, Li B, Li J, Wei S (2015) Fast film genres classification combining poster and synopsis. In: International conference on intelligent science and big data engineering. Springer, pp 72–81

%  Portolese G, Feltrim VD (2018) On the use of synopsis-based features for film genre classification. In: Anais do XV Encontro Nacional de Inteligencia Artificial e Computacional. SBC, pp 892–902

%  Portolese G, Domingues MA, Feltrim VD (2019) Exploring textual features for multi-label classification of portuguese film synopses. In: EPIA Conference on artificial intelligence. Springer, pp 669–681

%Eric Makita and Artem Lenskiy. A multinomial probabilistic model for movie genre predictions. arXiv preprint arXiv:1603.07849, 2016.

% Alex Blackstock and Matt Spitz. Classifying movie scripts by genre with a memm using nlp-based features, 2008.

% Ka wing Ho. Movies genres classification by synopsis, 2011

%Wehrmann, Jônatas, Maurício Armani Lopes, and Rodrigo Coelho Barros. "Self-attention for synopsis-based multi-label movie genre classification." The 31th International FLAIRS Conference, 2018, Brasil.. 2018.


% Other New

% Hanjalic, A., Xu, L.Q.: Affective video content representation and modeling. IEEE Transactions on Multimedia 7(1), 143–154 (2005)

% Xu, M., Chia, L.T., Jin, J.: Affective content analysis in comedy and
%horror videos by audio emotional event detection. In: IEEE International
%Conference on Multimedia and Expo (2005)

% Xu, M., Jin, J.S., Luo, S., Duan, L.: Hierarchical movie affective content analysis based on arousal and valence features. In: ACM Multimedia (2008)


==> tables/tab_app_incomprehensible_posters.tex <==
\begin{table}[] 
\centering
\caption{Misprediction by PrERDT on incomprehensible posters}
\label{tab:misclass1}
\begin{adjustbox}{width=0.49\textwidth}
\begin{tabular}{l | l | l}
\hline Poster sample & Actual genre & Predicted genre \\ \hline 
Fig. \ref{fig:incomprehensible}: \emph{i}    & Comedy, Drama, Fantasy     & Action, Adventure, Animation \\
Fig. \ref{fig:incomprehensible}: \emph{ii}    & Action, Drama, Mystery     & Horror, Sci-Fi, Thriller     \\
Fig. \ref{fig:incomprehensible}: \emph{iii}  & Drama, Mystery, Romance    & Action, Adventure, Sci-FI    \\
Fig. \ref{fig:incomprehensible}: \emph{iv}   & Action, Adventure, Comedy  & Drama, Horror, Romance       \\
Fig. \ref{fig:incomprehensible}: \emph{v}    & Action, Adventure, Fantasy & Drama, Horror, Mystery       \\
Fig. \ref{fig:incomprehensible}: \emph{vi}   & Drama, Romance             & Action, Horror               \\
Fig. \ref{fig:incomprehensible}: \emph{vii}  & Biography, Drama           & Action, Adventure, Sci-Fi    \\
Fig. \ref{fig:incomprehensible}: \emph{viii} & Adventure, Comedy, Fantasy & Drama, Horror, Mystery       \\
Fig. \ref{fig:incomprehensible}: \emph{ix}   & Comedy, Fantasy            & Drama, Mystery               \\
Fig. \ref{fig:incomprehensible}: \emph{x}    & Mystery, Thriller          & Comedy, Drama, Romance       \\
Fig. \ref{fig:incomprehensible}: \emph{xi}   & Biography, Drama           & Action, Adventure, Thriller  \\
Fig. \ref{fig:incomprehensible}: \emph{xii}  & Action, Drama, Sci-Fi      & Biography, Drama, Mystery    \\
Fig. \ref{fig:incomprehensible}: \emph{xiii} & Comedy, Drama, Fantasy     & Biography, Drama, Romance    \\
Fig. \ref{fig:incomprehensible}: \emph{xiv}  & Drama, Romance, Sci-Fi     & Biography, Crime, Drama      \\
Fig. \ref{fig:incomprehensible}: \emph{xv}   & Drama, Fantasy, Mystery    & Biography, Drama, Romance    \\
Fig. \ref{fig:incomprehensible}: \emph{xvi}  & Drama, Fantasy, Mystery    & Biography, Drama, Mystery   \\
\hline 
\end{tabular}
\end{adjustbox}
\end{table}
